Exploitability Minimization in Games and Beyond

Pseudo-games are a natural and well-known generalization of normal-form games, in which the actions taken by each player affect not only the other players' payoffs, as in games, but also the other players' strategy sets. The solution concept par excellence for pseudo-games is the generalized Nash equilibrium (GNE), i.e., a strategy profile at which each player's strategy is feasible and no player can improve their payoffs by unilaterally deviating to another strategy in the strategy set determined by the other players' strategies. The computation of GNE in pseudo-games has long been a problem of interest, due to applications in a wide variety of fields, from environmental protection to logistics to telecommunications. Although computing GNE is PPAD-hard in general, it is still of interest to try to compute them in restricted classes of pseudo-games. One approach is to search for a strategy profile that minimizes exploitability, i.e., the sum of the regrets across all players. As exploitability is nondifferentiable in general, developing efficient first-order methods that minimize it might not seem possible at first glance. We observe, however, that the exploitability-minimization problem can be recast as a min-max optimization problem, and thereby obtain polynomial-time first-order methods to compute a refinement of GNE, namely the variational equilibria (VE), in convex-concave cumulative regret pseudo-games with jointly convex constraints. More generally, we also show that our methods find the stationary points of the exploitability in polynomial time in Lipschitz-smooth pseudo-games with jointly convex constraints. Finally, we demonstrate in experiments that our methods not only outperform known algorithms, but that even in pseudo-games where they are not guaranteed to converge to a GNE, they may do so nonetheless, with proper initialization.

==> Exploitability Minimization in Games and Beyond (NeurIPS)/GNE.tex <==
\section{Generalized Nash Equilibrium}

\begin{theorem}
Suppose that $\constraints$ is non-empty-, compact-, convex-valued, and continuous and that $\objs$ is continuous, then the VI $(\constraints, \objs)$ has at least one solution.
\end{theorem}

Additionally, just any NE is a solution to VI, we have that that every abstract economy has a GNE which is a solution to some QVI problem, the proof follows similarly.

\begin{theorem}
A strategy profile $\action^* \in \actionspace$ is a GNE of  of an abstract economy $(\numplayers, \actions, \util)$ iff it it a solution to the QVI $(\actions, - \grad[\action] \util)$.
\end{theorem}
Finally, we have the following corollary which demonstrates the existence of GNE in abstract economies


\begin{corollary}
Every abstract economy $(\numplayers, \actions, \util)$ where $\util$ is continuously differentiable has at least one Nash equilibrium.
\end{corollary}

\begin{remark}
Note that, once again, the assumption of the marginal utility being continuous can be done away (leaving us with Arrow-Debreu's lemma on abstract economies \cite{arrow-debreu}) by replacing replacing the gradient operator with the subdifferential operator, in which case $\objs$ becomes a correspondence and the VI problem becomes a \mydef{generalized QVI}, for which similar existence results holds under similar continuity assumptions.
\end{remark}



% A tuple of strategy profiles $\action^*, \otheraction^* \in \actions(\action^*)$ is said to be a \mydef{Stackelberg-best-response equilibrium (SBRE)} if for all $\player \in \players$ and for all $\action \in \actions(\action^*)$, 
% \begin{align}
%     \min_{\action \in \actionspace : \actionconstr(\action) \geq \zeros} \max_{\otheraction \in \actions(\action)} \cumulregret(\action, \otheraction) \geq  \cumulregret(\action^*, \otheraction^*) \geq \max_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction)
% \end{align}
% Intuitively, an SBRE is \deni{Wtf am I trying to say here omg.}
% or equivalently if for all $\player \in \players$
% %
% \begin{align}
%     \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \regret[\player](\action[\player]^*, \otheraction[\player] ; \naction[\player]^*) \leq 0
% \end{align}




\begin{lemma}
Consider an abstract economy $(\numplayers, \actions, \util)$. Suppose that there exists a strategy profile $\action^* \in \actions(\action^*)$ such that $\max_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction) = 0$, then $\argmax_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction) $ corresponds to the set of GNE of the abstract economy $(\numplayers, \actions, \util)$.
\end{lemma}

\begin{proof}
We have:
\begin{align}
    \max_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction) &= 0\\
    \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \sum_{\player \in \players}  \left( \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) &= 0\\
    \sum_{\player \in \players} \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \left( \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) &= 0\\
    \sum_{\player \in \players}  \left( \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) &= 0
\end{align}
Since by \Cref{lemma:no_exploit_gne}, $\sum_{\player \in \players}  \left( \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) \geq 0$, we must have  that for all players $\player \in \players$:
\begin{align}
    \util[\player](\action^*) = \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)}  \util[\player](\otheraction[\player], \naction[\player]^*)  
\end{align}

That is, $\argmax_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)}  \util[\player](\otheraction[\player], \naction[\player]^*)$ is the set of best response of player $\player \in \players$ and that $\bigtimes_{\player \in \players} \argmax_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)}  \util[\player](\otheraction[\player], \naction[\player]^*)$ is the set of best-responses for all players which are fixed points of the abstract economy. 
\end{proof}


 


\begin{theorem}
Consider an abstract economy $(\numplayers, \actions, \util)$, and suppose that \Cref{assum:jointly_convex} holds and a GNE exists. Let $\cumulregret(\action, \otheraction) = \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])$, then 
any GNE of $(\numplayers, \actions, \util)$ is a Stackelberg equilibrium strategy $\action^*$ for the outer player in the following min-max game:
\begin{align}
    \min_{\action \in \actionspace: h(\action) \geq 0} \max_{\otheraction \in \actionspace:  \h(\otheraction[\player], \naction[\player]) \geq 0} \cumulregret(\action, \otheraction)
\end{align}
\end{theorem}

\begin{proof}
We have that $\min_{\action \in \actionspace: h(\action) \geq 0} \max_{\otheraction \in \actionspace:  h(\otheraction[\player], \naction[\player]) \geq 0} \cumulregret(\action, \otheraction) \geq 0$ by \Cref{lemma:no_exploit_gne}, and since a GNE $\action^* \in \actions(\action^*)$ exists, we must have that $\action^* \in \argmin_{\action \in \actionspace: \h(\action) \geq 0} \max_{\otheraction \in \actionspace:  \h(\otheraction[\player], \naction[\player]) \geq 0} \cumulregret(\action, \otheraction) $.
\end{proof}

Since games are special cases of abstract economies, we also obtain the following corollary which shows that any game is an instance of a min-max game.
\begin{corollary}
Consider a game $(\numplayers, \actionspace, \util)$ and suppose that a NE exists. Let $\cumulregret(\action, \otheraction) = \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])$, then 
% the set of GNE of $(\numplayers, \actionspace, \util)$ is equal to the set of SE of $(\actionspace, \actionspace, \cumulregret, \constr)$. That is, 
any NE of $(\numplayers, \actionspace, \util)$ is a Stackelberg equilibrium strategy $\action^*$ for the outer player in the following min-max Stackelberg game:
\begin{align}
    \min_{\action \in \actionspace} \max_{\otheraction \in \actionspace} \cumulregret(\action, \otheraction)
\end{align}
\end{corollary}







==> Exploitability Minimization in Games and Beyond (NeurIPS)/abstract.tex <==
\begin{abstract}
Pseudo-games are a natural and well-known generalization of normal-form games, in which the actions taken by each player affect not only the other players' payoffs, as in games, but also the other players' strategy sets. The solution concept par excellence for pseudo-games is the generalized Nash equilibrium (GNE), i.e., a strategy profile at which each player's strategy is feasible and no player can improve their payoffs by unilaterally deviating to another strategy in the strategy set determined by the other players' strategies. The computation of GNE in pseudo-games has long been a problem of interest, due to applications in a wide variety of fields, from environmental protection to logistics to telecommunications. Although computing GNE is PPAD-hard in general, it is still of interest to try to compute them in restricted classes of pseudo-games. One approach is to search for a strategy profile that minimizes exploitability, i.e., the sum of the regrets across all players. As exploitability is nondifferentiable in general, developing efficient first-order methods that minimize it might not seem possible at first glance. We observe, however, that the exploitability-minimization problem can be recast as a min-max optimization problem, and thereby obtain polynomial-time first-order methods to compute a refinement of GNE, namely the variational equilibria (VE), in convex-concave cumulative regret pseudo-games with jointly convex constraints. More generally, we also show that our methods find the stationary points of the exploitability  in polynomial time in Lipschitz-smooth pseudo-games with jointly convex constraints. Finally, we demonstrate in experiments that our methods not only outperform known algorithms, but that even in pseudo-games where they are not guaranteed to converge to a GNE, they may do so nonetheless, with proper initialization. \deni{Should we mention VE in the abstract?} \amy{probably, but how? where?}
\end{abstract}
% \deni{ATTN: DO NOT FORGET TO SAY VE INSTEAD OF GNE WHEN APPROPRIATE!!!}
%We provide convergence bounds to \samy{strategy}{action} profiles which are 1) stationary points of the exploitability of the pseudo-game in a large class of smooth\deni{I am saying this just to briefly mention that I am assuming that the payoff of the players are twice continuously differentiable} pseudo-games, and 2) GNE under additional assumptions on the payoffs of the players. Advantages of the methods presented in this paper, is 1) they are applicable to all smooth GNE problems with jointly convex constraints, 2) are fast, and 3) the output of these methods provide error bounds at no extra cost. Finally, we apply our algorithms to solve a class of benchmark pseudo-games, and Arrow-Debreu markets, a canonical example of a difficult pseudo-game. Our experiments suggest directions for improved exploitability minimization algorithms.


==> Exploitability Minimization in Games and Beyond (NeurIPS)/ack.tex <==
\begin{ack}
The ideas in this paper stemmed from conversations and seminars held during the Learning in Games workshop at the Simons Institute for the Theory of Computing.
This work was also supported by NSF Grant CMMI-1761546.
\end{ack}

==> Exploitability Minimization in Games and Beyond (NeurIPS)/arrow_debreu.tex <==
\section{Beyond Joint Convexity: The Example of Arrow-Debreu Markets}
Much of this paper has focused on jointly convex pseudo-games. Yet, most of the interesting applications for pseudo-games beyond this realm. We close our work with an algorithm to compute GNE beyond jointly convex domains, and provide empirical evidence of its efficacy on a canonical example of pseudo-game which is not jointly convex. We benchmark our algorithm to the most well-known algorithm to solve Arrow-Debreu markets, \mydef{t\^atonnement}, an auction-like algorithm. Before we present our results, let us recall that any pseudo-game can be written as the following ``quasi-optimization'' problem: 
$
    \min_{\action \in \actions(\action)} \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
$
Since the order of the minimum operations can be exchanged, we can decompose the outer minimization problem into $\numplayers$ minimization problems:
\begin{align}
    \min_{\action[1] \in \actions[1](\naction[1])} \min_{\action[2] \in \actions[2](\naction[2])}
    \hdots
    \min_{\action[\numplayers] \in \actions[\numplayers](\naction[\numplayers])}
    \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
\end{align}

The advantage of this reformulation is that it does away with the problem of simultaneously minimizing a function and solving for a fixed point problem, a problem for which no algorithms are known, and turns it into a sequential optimization problem. Even though such problems are in general NP-hard \cite{dempe2002foundations}, a local solution to such problems can often be found. This is quite desirable since very little is known on solving pseudo-games which are not jointly convex. More precisely, using the envelope theorem \cite{afriat1971envelope, milgrom2002envelope}, one can differentiate through each optimization problem to run a sequential gradient method which one would hope would converge to a stationary point of the exploitability. We note that although this approach seems very similar to that of backpropagation to obtain a direction of descent for neural network parameters, it is an inherently different method since backpropagation would make use of the implicit function theorem and the chain rule, while this approach calls for the computationally more appealing envelope theorem.

An \mydef{Arrow-Debreu (Exchange) economy model} consists of a finite set of $\numgoods$ goods, and $\numbuyers$ traders (i.e., agents/consumers). Every trader $\buyer \in \buyers$ has a set of possible consumptions $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}_+$, an endowment of goods $\consendow[\buyer] = \left(\consendow[\buyer][1], \dots, \consendow[\buyer][\numgoods] \right) \in \R^\numgoods$, a utility function $\util[\buyer]: \mathbb{R}^{\numgoods } \to \mathbb{R}$. We denote $\consumptions = \bigtimes_{\buyer \in \buyers} \consumptions[\buyer]$, and $\consendow = \left(\consendow[1], \hdots, \consendow[\numbuyers] \right)^T$. An Arrow-Debreu market is denoted by a tuple $(\util, \consumptions, \consendow)$ A \mydef{Walrassian equilibrium (WE)} is a tuple which consists of allocations $\allocation \in \R_+^{\numgoods \times \numbuyers}$, and prices $\price \in \R_+^\numgoods$ such that 1.~traders maximize utility: \\$\forall \buyer \in \buyers \ \ \ \allocation[\buyer]^*$ maximizes $\util[\buyer](\allocation[\buyer])$ over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$, 2.~the markets clear and goods that are not demanded are priced at 0, i.e., $ \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  \leq \sum_{\buyer = 1}^{\numagents} \consendow[\buyer]$ and $\price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \sum_{\buyer = 1}^{\numagents} \consendow[\buyer] \right) = 0$. Any Arrow-Debreu market can be formulated as a pseudo-game whose set of GNE is equal to the of WE of the original market \cite{arrow-debreu}. We provide a new pseudo-game formulation of Arrow-Debreu markets, whose exploitability is much easier to differentiate. 
	
\begin{theorem}
Consider the Arrow-Debreu market $(\util, \consumptions, \consendow)$, then any WE $(\allocation^*, \price^*)$, corresponds to a Stackelberg equilibrium strategy of the outer player $(\allocation^*, \price^*)$ in the following convex-concave min-max Stackelberg game:
\begin{align}
    \min_{(\allocation, \price) \in \consumptions \times \simplex[\numgoods] : \allocation \price \leq \consendow \price} \max_{(\Y, \q) \in \consumptions \times \simplex[\numgoods] : \Y \price \leq \consendow \price} \left(\q - \price \right)^T \left(  \sum_{\buyer \in \buyers} \allocation[\buyer] - \sum_{\buyer \in \buyers} \consendow[\buyer] \right) + \sum_{\buyer \in \buyers} (\consendow[\buyer] \cdot \price ) \left( \log(\util[\buyer](\y_{\buyer}))  - \log(\util[\buyer](\allocation[\buyer])) \right)
\end{align}
\end{theorem}


\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_arrow_debreu_linear.png}
         \caption{Linear Arrow-Debreu Market}
         \label{fig:linear_ad}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_arrow_debreu_cd.png}
         \caption{Cobb-Douglas Arrow-Debreu Market}
         \label{fig:cd_ad}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_arrow_debreu_leontief.png}
         \caption{Leontief Arrow-Debreu Market}
         \label{fig:leontief_ad}
     \end{subfigure}
        \caption{Convergence of sequential exploitability descent in Arrow-Debreu markets.
        % for \ref{fig:phase_zero_sum_affine} a game with one action, and 
        }
        \label{fig:ad}
\end{figure*}



==> Exploitability Minimization in Games and Beyond (NeurIPS)/checklist.tex <==
% \section*{Submission of papers to NeurIPS 2022}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Appendix A}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, details are discussed in conclusion, and experiments sections.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Assumptions are summarized in \Cref{assum:main}}
        \item Did you include complete proofs of all theoretical results? 
    \answerYes{Yes, all proofs can be found in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, code repo can be found here: \coderepo.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details can be found in section 5 and Appendix A.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{For experiments run multiple times, i.e., zero-sum convex constraints, exploitability always reached zero, and there was hence no error to report in all randomly initialized examples.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details can be found in Appendix A.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Details can be found in Appendix A}
  \item Did you mention the license of the assets?
    \answerYes{Details can be found in Appendix A}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> Exploitability Minimization in Games and Beyond (NeurIPS)/conclusion.tex <==
\section{Conclusion}

\if 0
%%% copied from the rebuttal !!!
Our main contribution is the observation that the exploitability-minimization problem can be recast as a simple and seemingly trivial min-max optimization problem (Observation 3.1). To the best of our knowledge we are the first to notice this equivalence. Some evidence in support of this claim is that otherwise the literature would have not have emphasized the arguably more complicated relaxation or Newton methods to overcome the nondifferentiability of exploitability.

*The strength of our paper lies in the simplicity of this previously unobserved min-max formulation, which allows us to provide an affirmative answer to Flam and Ruszczynski’s 20+-year-old conjecture [2] that projected gradient methods could be developed to minimize exploitability in pseudo-games.* We note that existing methods [1] make use of the exploitability concept to analyze algorithms that take alternative approaches, but they are not exploitability-minimization algorithms per se, as exploitability itself is not explicitly minimized.

More precisely, we solve for $\varepsilon$-GNE in convex-concave cumulative regret pseudo-games with jointly convex constraints (e.g., zero-sum, potential, Cournot, a large class of monotone pseudo-games and a novel class of bilinear pseudo-games, namely those with with convex second-order approximations (see Proposition (4c) of [2])) in $O(\frac{\log(\varepsilon)}{\varepsilon})$ iterations (Algorithm 1 - EDA, Theorem 3.4). We also obtain convergence to an $\varepsilon$-stationary point of the exploitability (Algorithm 2 - ADA, Theorem 4.2) more generally in all Lipschitz-smooth pseudo-games with jointly convex constraints. We note that ADA is also guaranteed to converge to $\varepsilon$-GNE in the class of convex-concave cumulative regret pseudo-games with jointly convex constraints at the same rate (Corollary of Theorem 4.2 and Theorem 4.3). These results, in our opinion, are very interesting, as combined with the $O(\frac{1}{\varepsilon})$ lower bound complexity of Nash equilibrium in two-player games [3], they reveal that the complexities of solving zero-sum, potential, a large class of monotone pseudo-games, and a class of bilinear pseudo-games are all the same as those of the corresponding *games*!

EDA is thus an optimal algorithm, which achieves the same convergence rate as AMPQP in pseudo-games in which the latter converges (i.e., monotone pseudo-games with jointly affine constraints). Further, its convergence guarantees extend beyond monotone settings to a class of bilinear pseudo-games for which AMPQP is not guaranteed to converge. Similarly ADA converges, albeit at a slightly slower rate, in the class of pseudo-games for which AMPQP is guaranteed to converge, and it more generally converges in all Lipschitz-smooth pseudo-games with jointly convex constraints to an $\varepsilon$-stationary point of the exploitability. Further, as we demonstrate experimentally, ADA can converge to an $\varepsilon$-GNE with suitable initialization. This makes ADA the first algorithm to solve for the $\varepsilon$-GNE (where $\varepsilon$ is equal to the value of the exploitability at the stationary point of the exploitability) of Lipschitz-smooth pseudo-games—and, as a result, the $\varepsilon$-Nash equilibria of Lipschitz-smooth games, for which, as far as we are aware, such broad convergence guarantees are not known. The main tool we use in proving the convergence of ADA is a novel parametric Moreau envelope theorem (Theorem 4.1), which is likely valuable as an optimization tool in other applications as well.

All in all, our results 1) improve upon the state-of-the-art by extending polynomial-time convergence guarantees to a class of pseudo-games beyond monotone, and 2) provide a general approach to approximate, with convergence guarantees, solutions to Lipschitz-smooth pseudo-games with jointly convex constraints, which, as far as we are aware, is the first result of its kind.
\fi

\amy{don't forget to emphasize: we are the first ones to bring into the min-max literature the use of the projected gradient operator, which allows us to obtain a nice and clearly interpretable convergence theorem, something other works are not able to do.}

In this paper, we provide an affirmative answer to an open question first posed by \citeauthor{flam1994gne}  \cite{flam1994gne},
%(Section 1)
who suggested that projected gradient methods could be developed to minimize exploitability in pseudo-games. Although some existing methods \cite{facchinei2010generalized} make use of the exploitability concept to analyze algorithms that take alternative optimization approaches, we know of none that are exploitability-minimization algorithms per se, as exploitability itself is not explicitly minimized.
Our main contribution is the observation that the exploitability minimization problem can be recast as a simple and seemingly trivial min-max optimization problem (\Cref{obs:exploit_min_to_min_max}).
Our analysis effectively extends the class of games which can be solved as potential games, since the exploitability can be seen as a potential for any game.

%\amy{i don;t think i understand this phrase. i would assume that the class of games that can be solved as potential games is precisely the class of potential games. is it not?} \deni{A game can be a potential game but it might stil not be solvable as such because the potential is not easily optimizable.} \amy{do you have other examples, besides a typical non-zero-sum game for which we use exploitability as our potential? if so, please give one. thanks.}\deni{I am not sure I totally understand but if I understand what you are asking correctly, the monotone games presented in the experiments section is an example of this.}

We provide a definition of stationarity for exploitability via the gradient mapping operator from proximal theory, and we use this definition to characterize the limit points of our algorithms.
Our characterization relies on novel proof techniques inspired by recent analyses of algorithms for min-max optimization problems \cite{nouiehed2019solving}, as well as a parameterized version of Moreau's envelope theorem, which may be of independent interest.
%\amy{what does it mean to ``incorporate an operator into a perspective?''} 
This approach, which takes advantage of the structural properties of exploitability, allows us to rigorously analyze an algorithm that converges to stationary points of the VE exploitability in all Lipschitz-smooth pseudo-games with jointly convex constraints, and obtain algorithms which are orders of magnitude faster than known min-max optimization algorithms for similar types of problems.
%
To summarize, our results 1.~extend known polynomial-time convergence guarantees to VEs, and thus GNEs, to a class of pseudo-games beyond monotone, and 2.~provide a general approach to approximate, with convergence guarantees, solutions to Lipschitz-smooth pseudo-games with jointly convex constraints.
%\sdeni{, which, as far as we are aware, is the first result of its kind}{}.\amy{do we need to say here that it is the first result of its kind. we needed that in the rebuttal, but i'm not sure it is still needed.}\deni{I don't think it's necessary I feel like it sounds arrogant!}\amy{exactly!}

The design of efficient algorithms for constrained non-convex-concave min-max optimization problems is an open problem.
The literature thus far has focused on problems in which only the variable to be maximized is constrained \cite{nouiehed2019solving, jin2020local, lin2020gradient}.
Our techniques may provide a path to solving non-convex-concave min-max optimization problems in entirely constrained domains, since our algorithms solve a non-convex-concave optimization problem 
%%% SPACE
%in which
where both variables are constrained.


\if 0

\samy{}{The methods we propose in this paper take the exploitability-minimization perspective, reinterpreting GNEP as a min-max optimization problem of the cumulative regret, which gives rise to efficient and intuitive algorithms.}

At a high-level, our methods reformulate the exploitability quasi-minimization problem as a min-max Stackelberg game \cite{stackelberg1934marktform, goktas2021minmax}.
Our results provide convergence bounds to a stationary point of the exploitability for the largest class of pseudo-games 
%with jointly convex constraints
yet studied in the literature.
Additionally, we show that under suitable conditions on the problem, our method converges to a GNE.

\deni{Next two sentences to potentially edit/delete.} \sdeni{}{We also provide an extension of our methods to handle pseudo-games with joint constraints that are not necessarily jointly convex. We demonstrate via experiments that our algorithm converges to a GNE which seems to suggest that in practice our method often converges to GNEs, even in classes of problems for which it is not guaranteed to converge at all!}
\deni{Two contributions here: For the GNE convergence literature, we provide an applicable method and provide convergence bounds; for the newer bound literature, we enlargen the class of problems in which we converge.}
\fi


\if 0
We have considered exploitability minimization in pseudo-games and have proposed fast and universal algorithms to compute or approximate GNE in a large class of problems. Our theoretical guarantees go above and beyond the known convergence complexities of GNE in pseudo-games. %Finally, we have also ran a series of experiments on Arrow-Debreu markets which have suggested that our methods' efficacy extend beyond the scope of the theory displayed in this paper.
Future work should aim to explore different strongly-convex regularizers for different games in an effort to obtain more efficient exploitability-minimization algorithms.
\fi


==> Exploitability Minimization in Games and Beyond (NeurIPS)/experiments.tex <==
\section{Experiments}\label{sec:experiments}

\deni{In this last section I stuck to ``GNE'' rather than VE because the Michael Jordan paper computes a GNE, not a VE (although I think they are actually computing a VE)}\amy{are you sure? i think we should be more precise, esp. if you think that's what they are doing anyway. why propagate their mistake?}

In this section, we report on experiments %with simulated pseudo-games
that demonstrate the effectiveness of our algorithms as compared to others that were also designed to compute GNE.
We present numerical results on benchmark psuedo-games that were studied empirically in previous work \cite{raghunathan2019game}: %1) two-player zero-sum bilinear pseudo-games with jointly affine constraints; 
%2) two-player zero-sum bilinear pseudo-games with jointly convex constraints; 
1) monotone pseudo-games with affine constraints and 2) bilinear pseudo-games with jointly convex constraints.%
\footnote{We describe additional experiments in the supplemental work, with two-player zero-sum bilinear pseudo-games with jointly affine constraints and two-player zero-sum bilinear pseudo-games with jointly convex constraints. The results are not qualitatively different than those presented here.
All our code can be found on \coderepo.}
We compare our algorithms to the \mydef{accelerated mirror-prox quadratic penalty method} (AMPQP), the only GNE-finding algorithm with theoretical convergence guarantees \emph{and rates} \cite{jordan2022gne}.%
\footnote{We note that we are not reporting on our results with the Accelerated Mirror-Prox Augmented Lagrangian Method (AMPAL), another method studied in the literature with the convergence rates as AMPQP, because we found this algorithm to be unstable on our benchmark pseudo-games.}
For the AMPQP algorithm, we use the hyperparameter settings derived in theory when available, and otherwise conduct a grid search for the best ones.
%In all of our experiments, \EDA{} and \ADA{} converge to a GNE.
We compare the convergence rates of our algorithms to that of AMPQP, which converges at the same rate as \EDA, but slower than \ADA, in settings in which it is guaranteed to converge, i.e., in monotone pseudo-games.

In the monotone pseudo-games, for \EDA{} we use a constant learning rate of $\learnrate[ ] = 0.02$, while for \ADA{} we use the constant learning rates of $\learnrate[\action] = 0.02$ and $\learnrate[\action] = 0.05$. These rates approximate the Lipschitz-smoothness parameter of the pseudo-games.
In the bilinear pseudo-games, we use the theoretically-grounded (\Cref{thm:eegda}) learning rate of $\learnrate[ ] = \nicefrac{1}{\left\|\bm{Q}\right\|}$ for \EDA{}, and $\learnrate[\action] =\left\|\bm{Q} \right\| + \frac{\left\|\bm{Q} \right\|^2}{\regulparam}$ and $\learnrate[\otheraction] = \nicefrac{1}{\left\|\bm{Q} \right\|}$ for \ADA{}. 
In both settings, we use a regularization of $\regulparam = 0.1$ for \ADA, which we found by grid search.
Likewise, in our implementation of AMPQP, 
%facing a lack of theoretical parameter choice
grid search led us to initialize $\beta_0 = 0.01, \gamma = 1.05, \alpha = 0.2$ in both settings.%
\footnote{As suggested by \citeauthor{jordan2022gne} \cite{jordan2022gne}, we replaced the convergence tolerance parameter $\delta$, with the number of iterations for which the accelerated mirror-prox subroutine \cite{chen2017accelerated} was run.
Then, at each iteration of AMPQP, this parameter was increased by a factor of $\gamma$ of AMPQP.} 
Additionally, because the iterates generated by AMPQP are not necessarily feasible, we projected them onto the feasible set of actions, so as to avoid infinite exploitability.
This heuristic improved the convergence rate of AMPQP significantly.
The first iterate for all methods was common, and initialized at random.

\paragraph{Monotone Games with Jointly Affine Constraints}

%Next, we turn our attention to 
We begin by experimenting with monotone games with jointly affine constraints, the largest class of pseudo-games for which convergence rates exist for AMPQP.
In particular, we consider norm-minimization pseudo-games with payoff functions $\util[\player](\action) = - \left\| \sum_{\player \in \players} \action[\player] - \s_\player \right\|$, for all players $\player \in \players$, and for some randomly initialized shifting factors $\s_\player$, as well as jointly affine constraints $\constr[ ](\action) = 1 - \sum_{j \in [\numactions]} \action[1][j] - \sum_{i \in [\numactions]} \action[2][j]$, with action spaces $\actionspace[\player] = [-10, 10]^\numactions$, for all players $\player \in \players$.
Although norm-minimization games are trivial, in the sense that they can be solved in closed form, this is not the case for pseudo-games; on the contrary, they form a bedrock example for monotone pseudo-games (\cite{facchinei2010generalized}, Example 1).

In \Cref{fig:phase_monotone_affine}, we observe that all three algorithms converge to a GNE.
Interestingly, EDA and ADA find distinct GNEs from AMPQP, which is not entirely surprising, as AMPQP is not an exploitability minimization algorithm.
%However, we also observe convergence for EDA{} and \ADA{} in all \samy{randomly initialized examples}{of our experiments}, even though monotone pseudo-games are not convex-exploitability games.
%That said, for any monotone game one can build an approximate pseudo-game by replacing the payoff function functions of the players by their first-order Taylor approximation to obtain a convex exploitability \cite{von2009optimization}. In the case of norm-minimization games, this approximate game is very close to the original game since the payoff functions of the players has a very small Lipschitz-smoothness constants.\amy{did you build this approximate pseudo-game?}\deni{no!}
%As a result,\amy{i don't see how this can follow if you didn't use that approximation procedure} the algorithms converge to a GNE globally, i.e., we observed convergence \samy{for any randomly initialized first iterate in our experiments}{regardless of initial conditions, in all experiments}.
Although all the algorithms eventually find a GNE, exploitability does not decrease monotonically (\Cref{fig:exploit_monotone_affine}); on the contrary, it increases before eventually decreasing to zero.
Convergence to a GNE is expected for AMPQP, as per the theory.
%which is guaranteed to converge to a GNE this class of pseudo-games.
\EDA, however, is not guaranteed to converge to a GNE in pseudo-games beyond convex exploitability; yet, we still observe convergence, albeit at a slower rate than AMPQP or \ADA.
Likewise, \ADA{} converges to a GNE, although it is again not guaranteed, much faster than AMPQP.
%These experiments also highlight an advantage of \ADA{} over AMPQP: even in monotone games where AMPQP is guaranteed to converge to a GNE, \ADA{} converges much faster.

\begin{figure}[!t]
     \begin{subfigure}[b]{0.24\textwidth}
     \centering
         \includegraphics[width=\textwidth]{graphs/phase_halfspace_monotone.png}
         \caption{Phase portrait for a 2 player monotone game with $\numactions = 1$ }
         \label{fig:phase_monotone_affine}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_halfspace_monotone.png}
         \caption{Exploitability for a 5 player monotone game with $\numactions = 10$}
         \label{fig:exploit_monotone_affine}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/phase_ball_bilinear.png}
         \caption{Phase portrait for bilinear general-sum pseudo-game with $\numactions = 1$}
         \label{fig:phase_bilinear_convex}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_halfspace_bilinear.png}
         \caption{Exploitability for a bilinear general-sum pseudo-game; $\numactions = 10$}
         \label{fig:exploit_bilinear_convex}
     \end{subfigure}
        \caption{Convergence in monotone and bilinear general-sum pseudo-games.
        % for \ref{fig:phase_zero_sum_affine} a game with one action, and 
        }
        \label{fig:bilinear_monotone}
\end{figure}


\paragraph{Bilinear General-Sum Games with Jointly Convex Constraints}

Second, we consider the class of two-player general-sum games with jointly convex constraints with payoff functions 
$
    \util[1](\action) = \action[1]^T \bm{Q}_1 \action[2], \util[2](\action) = \action[1]^T \bm{Q}_2 \action[2],
    \constr[ ](\action) = 1 - \left\| \action \right\|_2^2,
    \actionspace[1] = \actionspace[2] = [-10, 10]^\numactions
$. 
Such games are not monotone, and hence AMPQP is not guaranteed to converge in theory. 
%
In \Cref{fig:phase_bilinear_convex}, we see that convergence is not guaranteed empirically either; shown is a sample run in which \ADA{} and \EDA{} converge, while AMPQP exhibits erratic behavior.
Non-convergence for AMPQP was observed in 93 of the 100 experiments run.
In fact, even though AMPQP gets very close a GNE (\Cref{fig:exploit_bilinear_convex}), i.e., zero exploitability, it does not stabilize there.
%as the algorithm is not necessarily locally stable around GNEs, 
%we observe erratic behavior.
We likewise found that \ADA{} and \EDA{} do not converge to a GNE from all random initializations.
In such cases,
% \amy{we need to say somewhere that this happened in far fewer than 93/100 experiments! and maybe that restarting AMPQP didn't help!}\deni{Let me run it an check what are the numbers!}
we restarted the algorithms with a new random initialization; this process lead to on average 11 restarts  for \EDA{} and 10 restarts for \ADA, meaning both algorithms converged to a GNE within this window.
%Perhaps in future work, we can develop heuristics which search for optimal initializations of exploitability-minimization methods.


==> Exploitability Minimization in Games and Beyond (NeurIPS)/intro.tex <==
% \amy{consider describing the whole story in terms of potential games, where the potential of interest is exploitability.}\deni{Although I think this is the correct way to see things I think rephrasing story in this term distracts the reader from the main goal of this paper: How to minimize exploitability efficiently. That said, i think this needs to be added into the conclusion! What do you think?} \amy{yes, please add to the conclusion if you have not already}

\section{Introduction}

Nash equilibrium \cite{nash1950existence} is the canonical solution concept used to predict the outcome of models of rational agents known as games.
% which has given rise to much of game theory
% \samy{has proven to be a revolutionary invention in a variety of fields from machine learning, to economics.}{}\amy{you cannot make claims as outlandish/extreme as this without backing them up by a ton of references}
A \mydef{game} comprises a set of players, each of whom simultaneously chooses a strategy (or action) from a strategy set, and then receives a payoff based on all the players' choices.
A \mydef{Nash equilibrium (NE)} is a strategy profile, i.e., a collection of strategies, one per player, from which no player can improve their payoff via a unilateral deviation.

Recently, the literature on NE has expanded beyond classic economic applications to the question of its computation, a problem known as the \mydef{Nash equilibrium problem (NEP)} \cite{osborne1994course, AGT-book}.
% \amy{add citation}
Unfortunately, it is unlikely that there exists an efficient algorithm to compute NE, as NEP is PPAD-complete, i.e., NEP is equivalent 
%\deni{PPAD-hard, means at least as hard as the problem in PPAD, i.e., every problem in PPAD reduces to it, PPAD complete means the other direction as well}
to the problem of computing solutions to a class of fixed-point problems known as PPAD \cite{papadimitriou1994complexity}, which are believed to be computationally intractable \cite{chen20053, chen2006settling, daskalakis2009complexity}.
Nonetheless, there has been a great deal of recent progress developing \emph{efficient\/} algorithms to compute NE in special classes of games, such as two-player zero-sum
\cite{tseng1995variational, nesterov2006variational, gidel2020variational, mokhtari2020convergence, ibrahim2019lower, zhang2020, lin2020near, alkousa2020accelerated, juditsky2011first, hamedani2018primal, zhao2019optimal, thekumparampil2019efficient, ouyang2018lower, nemirovski2004prox, nesterov2007dual, tseng2008accelerated, sanjabi2018stoch, nouiehed2019solving, lu2019block, jin2020local, ostrovskii2020efficient, lin2020gradient, zhao2020primal, rafique2019nonconvex}, potential \cite{monderer1996potential, sandholm2001potential, durand2016complexity}, and monotone (or, more generally, variationally stable) games \cite{nesterov2006solving, cai2022tight, malitsky2015projected, gorbunov2022extragradient,  tatarenko2019learning, he2002new, malitsky2014extragradient}.
Interest in two-player zero-sum games, for example, stems in part from emerging applications in machine learning, e.g., the training of GANs \cite{goodfellow2014gan, creswell2018gans}.

A natural generalization of games are \mydef{pseudo-games} or \mydef{abstract economies}, first introduced by \citeauthor{arrow-debreu} \cite{arrow-debreu} in the context of markets, in which the actions taken by each player affect not only the other players' payoffs, as in games, but also the other players' strategy sets.
In other words, players (simultaneously) take actions that can restrict the other players' strategy sets.
Such a model is not technically a game, giving rise to the pseudo-game terminology.
Pseudo-games generalize games, and hence are even more widely applicable.
Some recently studied applications include adversarial classification \cite{bruckner2012nash, bruckner2009nash}, energy resource allocation \cite{hobbs2007power, wei1999power}, environmental protection \cite{breton2006game, Krawczyk2005environ}, cloud computing \cite{ardagna2017cloud, ardagna2011cloud}, adversarial classification, ride sharing services \cite{ban2019rides}, transportation \cite{stein2018transport},  wireless and network communication \cite{han2011wireless, pang2008distributed}.
%For illustrations of these applications, we refer the reader to survey papers on \samy{GNEs}{pseudogames} \cite{facchinei2007generalized, facchinei2010generalized, fischer2014GNE}.

\if 0
\amy{actually, i believe those examples make it just as important to compute Nash. so far, only the A-D market application has convinced me that it is important to compute GNE.}\deni{This is not true!!! The applications I am citing actually use GNE not NE, I do not think we should move them!!! Remember for instance the telecomunication example from the facchinei paper}\amy{i know that. that is not what i am saying. i am saying that 10-20 years ago people were writing papers about the same application areas, and claiming that games were the right model, and accordingly Nash equilibrium was the solution concept par excellence for these applications.}
\fi

The solution concept par excellence for pseudo-games is the \mydef{generalized Nash equilibrium (GNE)} \cite{arrow-debreu, facchinei2010generalized, fischer2014GNE}, i.e., a strategy profile at which each player's strategy is feasible and no player can improve their payoffs by unilaterally deviating to another strategy in the strategy set determined by the other players' strategies.
The aforementioned applications speak to the importance of developing algorithms that can approximate GNEs efficiently in the largest class of pseudo-games possible.
% \sdeni{}{As the \mydef{generalized Nash equilibrium problem (GNEP)} generalizes the NEP, and has many applications as aforementioned, developing algorithms that can approximate GNEs efficiently in the largest class of pseudo-games possible is of great importance.}
%\amy{i think the sentence that was there before, and which i uncommented out, is better. i don't think i am one to proclaim a problem of great importance. i prefer the earlier sentence b/c it blames the applications for asserting the importance of the problem!} \deni{Fair enough!}
Work in this direction, on the \mydef{generalized Nash equilibrium problem (GNEP)}, is progressing; see, for example, 
\cite{facchinei2009generalized, facchinei2010generalized, facchinei2011computation, paccagnan2016distributed, yi2017distributed, couzoudis2013computing, dreves2017computing, von2009optimization, tatarenko2018learning, dreves2016solving, von2012newton, izmailov2014error, fischer2016globally, pang2005quasi, facchinei2011partial, fukushima2011restricted, kanzow2016multiplier, kanzow2016augmented, kanzow2018augmented, ba2020exact}.
Nonetheless, there are still few, if any \cite{jordan2022gne}, GNE-finding algorithms with computational guarantees, even for restricted classes of pseudo-games.

% the \textbf{Nikoida-Isoda potential function} \cite{}, \emph{a.k.a.\/}
\textbf{Exploitability}, or the Nikoida-Isoda potential \cite{nikaido1955note}, is defined as the sum of the players' payoff-maximizing unilateral deviations w.r.t.\ a given strategy profile.
%
Minimizing exploitability is a logical approach to computing GNE, especially in cases where exploitability is convex, such as in the pseudo-games that result from replacing each player's payoff function in a monotone pseudo-game by a second-order Taylor approximation \cite{flam1994gne}.
When the players' payoffs are also Lipschitz-smooth and strongly concave (in their own action), this approximation can be quite good, because the error in the %second-order Taylor 
approximation will be bounded by the Lipschitz-smoothness and strong concavity constant.
\emph{Minimizing exploitability can thus be an effective way of finding GNEs in pseudo-games; however, to our knowledge, no convergence rates for this approach are known, and few methods have been proposed for pseudo-games whose exploitability is non-convex.}

%All these applications suggest the \sdeni{}{far-reaching} power of minimizing exploitability in GNE computation,\amy{very general approach, works ``universally''}

In this paper, we develop efficient
exploitability-minimization algorithms that converge to variational equilibrium (VE), a refinement of GNE, exactly 
%\deni{Maybe the convergence language is better since asymptotically we are guaranteed to converge to an exact GNE in convex-concave cumulative regret games.}
in a large class of pseudo-games with jointly convex constraints (which includes, but is not limited to, two-player zero-sum, $\numplayers$-player pairwise zero-sum, and a large class of monotone and bilinear pseudo-games, as well as Cournot oligopoly games); and approximately, in Lipschitz-smooth pseudo-games with jointly convex constraints, where exact computation is intractable.
Our algorithms apply not only to games with discrete action spaces but also to games with continuous action spaces; previous exploitability-minimization algorithms concern only finite games \cite{lockhart2019exploit, gemp2021sample}.
%\samy{, and prove convergence to approximate GNEs in almost all pseudo-games of practical interest}{}.\amy{which are these? Lipschitz-smooth? i would be surprised. that would mean the Nash PPAD result doesn't really matter b/c it doesn't apply to games of practical interest. that seems like a big claim.}
% the sum across all players of the differences between the utility of all players playing one strategy profile, and one player deviating to a strategy in the other strategy profile while other players' strategies stay fixed

The \mydef{cumulative regret} of two strategy profiles is defined as the sum, across all players, of the change in utility due to unilateral deviations from one strategy profile to the other.
Our algorithms and their analysis rely on the following key insights: assuming jointly convex constraints (i.e., symmetric and convex-valued joint constraint correspondences) the exploitability-minimization problem is equivalent to solving a cumulative regret min-max optimization problem, %(with independent constraint sets)
which although non-convex-concave in general can nonetheless be solved by \mydef{gradient descent ascent (GDA)} methods%
\footnote{When the objective function is convex-concave,
%a min-max Stackelberg game reduces to a (simultaneous-move) min-max game,
a saddle point is guaranteed to exist, in which case this optimization problem can be solved using simultaneous-GDA-style algorithms (e.g., \cite{nemirovski2004prox, korpelevich1976extragradient, nedic2009gda}).} \cite{nouiehed2019solving, goktas2021minmax} using a parametric variant of Moreau's envelope theorem that we introduce (\Cref{thm:moreau_envelope}).
We apply this logic to develop two algorithms for Lipschitz-smooth pseudo-games with jointly convex constraints.
\emph{To the best of our knowledge, this makes ours the first exploitability-minimization methods with convergence rate guarantees in this class of pseudo-games.}

The first (\EDA{}; \Cref{alg:egda_cumul_regret}) is an extragradient method that converges in average iterates to an $\varepsilon$-VE, and hence an $\varepsilon$-GNE, in $O(\nicefrac{1}{\varepsilon})$ iterations in pseudo-games with convex-concave cumulative regret, where $\varepsilon$ is the exploitability of the game (\Cref{thm:eegda}).
This class of pseudo-games includes zero-sum, potential, Cournot, a large class of monotone pseudo-games, and a class of bilinear pseudo-games, namely those with convex second-order approximations.
%
%\deni{Note this algo converges in games with convex-concave cumulative regret which are convex exploitability games, but the other way round is not necessarily true, i.e., convex exploitability does not imply convex-concave cumulative regret.}
%
Our second algorithm (\ADA; \Cref{alg:cumul_regret}) is a nested GDA algorithm, 
%which in an inner loop computes an approximate best-response strategy profile to the current outer loop strategy profile, and then uses this approximate best response in an outer loop to improve the outer loop's strategy profile.
whose best iterate converges  more generally to a stationary point of (regularized) exploitability in all Lipschitz-smooth pseudo-games with jointly convex constraints at the slightly slower rate of $O(\nicefrac{\log(\nicefrac{1}{\varepsilon})}{\varepsilon})$  (\Cref{thm:convergence_stationary_approx}).
When the (regularized) exploitability is additionally invex, our method also converges to a GNE in best iterates at the same rate.
This convergence can be strengthened to convergence in last iterates in $O(\log(\nicefrac{1}{\varepsilon})^2)$ iterations in strongly-convex exploitability pseudo-games and in a certain class of pseudo-games with non-convex exploitability
(\Cref{thm:pl_convergence}).

% \amy{what is an example of an important class of pseudo-games where the constraints are jointly convex? i know in our exp'ts we just use toy games, but in addition to moving to the non-jointly convex setting, we also want to say that in the future we will apply our current methods to more realistic jointly convex pseudo-games. so can we describe one? and explain why joint convexity makes sense for that application? this sort of story would be analogous to the claim that zero-sum games are important b/c of GANs. same idea here. why are jointly convex pseudo-games important? what is our killer app for this class? what is our justification for studying this problem.}\deni{There are quite a few, will pull them out and add a paragraph}

%a way to model resource allocation as games
Pseudo-games with jointly convex constraints are of interest in decentralized resource allocation problems with feasibility (e.g., supply) constraints.
% where a policy maker wants to allocate a set of resources across different agents.
% When the problem is centralized, %i.e., the policymaker decides the allocation of resources to each agent, 
% the
Feasibility constraints are almost always joint, and often also jointly convex, since we generally require the sum of the allocations to be less than or equal to the supply.
One of the many examples of such pseudo-games is wireless and network communication, where agents communicate packets across a shared network, with limited capacities \cite{han2011wireless}.
% decentralized:
% 
% centralized:
%electricity companies decide how to distribute resources among their customers \cite{hobbs2007power, wei1999power}.
The experiments we run in this paper suggest that our algorithms have the potential to yield improved solutions to such pseudo-games as compared to other known approaches, and thus open up avenues for practical applications of our work in the future.

% \amy{say something about experiments. theory papers might eek by, but NeurIPS is historically about experimental work}

% \deni{do you think it is confusing that in the prelims I define the pseudo-game to have jointly convex constraints, but I do not call it jointly convex pseudo-game. I am worried that maybe people might be thinking the payoff functions are concave in all players' variables.}


==> Exploitability Minimization in Games and Beyond (NeurIPS)/jointly.tex <==

In recent years, a variety of methods have been developed that could be applied to finding stationary points of the exploitability \cite{thekumparampil2019efficient, nouiehed2019solving, lu2019block, jin2020local, rafique2019nonconvex}.
Using the most efficient of these methods, one could obtain convergence to an $\varepsilon$-stationary point of the exploitability in  $O(\nicefrac{1}{\varepsilon^6})$ iterations
%at best
\cite{thekumparampil2019efficient}. However, as we will see,
%\amy{do we actually show this?}\deni{we show it in the sense that we provide algos which can compute a stationary point in a number of iterations that is 5 orders of magnitude smaller} 
this rate would be very slow, and the convergence metric, not very strong, e.g., convergence in expected iterates.
Instead, we demonstrate how to leverage the structure of the exploitability-minimization problem
%$\min_{\action \in \actions} \exploit (\action)$ 
%\max_{\otheraction \in \actions} \cumulregret(\action, \otheraction)
to obtain much faster convergence rates.

\deni{what do you prefer as language, regularized cumulative regret vs. augmented cumulative regret?}\amy{regularized, but that's cuz i'm a bit closer to the ML community than opt'n. but...our algo is called Augmented! so, maybe augmented is better?}

Unfortunately, the exploitability associated with the min-max 
%Stackelberg game
characterization of pseudo-games with joint constraints is non-differentiable in general.
This fact poses an obstacle when trying to design efficient algorithms that find its stationary points.
However, by exploiting the structure of cumulative regret, we can regularize it to obtain a smooth objective.
%\sdeni{In particular, for all $\action^* \in \argmin_{\action \in \actions} \max_{\otheraction \in \actions} \cumulregret(\action, \otheraction)$, there exists $\otheraction^* \in \max_{\otheraction \in \actions} \cumulregret(\action^*, \otheraction)$ such that $\action^* = \otheraction^*$.}
Observe the following: if $\action^* \in \argmin_{\action \in \actions} \max_{\otheraction \in \actions} \cumulregret(\action, \otheraction)$, then $\action^* \in \argmax_{\otheraction \in \actions} \cumulregret(\action^*, \otheraction)$. 
In other words, $\otheraction^* = \action^*$ is a solution to the inner maximization problem.
As a result, we can penalize exploitability in proportion to the distance between $\action$ and $\otheraction$, while still ensuring that this penalized exploitability is minimized at a VE.
We thus optimize the $\regulparam$-\mydef{regularized cumulative regret} $\cumulregret[\regulparam]: \actionspace \times \actionspace \to \R$, defined as $\cumulregret[\regulparam] (\action, \otheraction) \doteq \cumulregret (\action, \otheraction) - \frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2$, whose associated \mydef{$\regulparam$-regularized exploitability} $\exploit[\regulparam]: \actionspace \to \R$ is given by
$\exploit[\regulparam] (\action) = \max_{\otheraction \in \actions} \cumulregret[\regulparam] (\action, \otheraction)$.
\citeauthor{von2009optimization} show that a strategy profile $\action^*$ has no $\regulparam$-regularized-exploitability, i.e., $\exploit[\regulparam](\action^*) = 0$, iff $\action^*$ is a VE for all $\regulparam > 0$ (Theorem 3.3 \cite{von2009optimization}). 
% $\exploit[\regulparam]$ %$\argmax_{\otheraction \in \actions} \cumulregret[\regulparam](\action, \otheraction)$  is a singleton-valued correspondence \amy{are we using this second fact somewhere? maybe in the proofs? i am not seeing where we invoke it in the paper?}\deni{In the proofs!} .

% \if 0
% Next, we present an important theorem, which
% %builds upon the results of \citeauthor{von2009optimization} \cite{von2009optimization}, and 
% is key to deriving an algorithm that converges fast to stationary points of the exploitability.
% %in all Lipschitz-smooth pseudo-games with jointly convex constraints.
% \fi
%The following theorem tells us that for $\regulparam > 0$, the set of Stackelberg equilibria of the non-convex-concave min-max Stackelberg game $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulregret[\regulparam](\action, \otheraction)$, is equal to the set of VE of the pseudo-game associated with $\cumulregret$, and characterizes the smoothness properties of $\regulparam$-regularized exploitability.
%The novelty of the following theorem over Theorems 3.3 and 3.5 of

To better understand the smoothness properties of the regularized exploitability, we present the \mydef{parametric Moreau envelope}, a Moreau envelope \cite{moreau1965proximite} in which the objective function is a function of the point w.r.t.\ which we regularize the objective function, which in our case is cumulative regret.
% Additionally, 
%it turns out that 
% as we show next, 
%$\exploit[\regulparam]$ 
% the  $\regulparam$-regularized-exploitability corresponds to t
Our next theorem is a generalization of the Moreau envelope theorem \cite{moreau1965proximite}, which shows that $\regulparam$-regularized exploitability is Lipschitz-smooth, by allowing us to see $\exploit[\regulparam]$ as a parametric Moreau envelope for $\cumulregret$, an observation which to our knowledge has not been made in previous work.
% , which implies that it is Lipschitz-smooth,.
%\samy{whose gradient is given by $\grad[{\action[\player]}] \exploit[\regulparam](\action) =  \sum_{\player \in \players}  \left[ \grad[{\action[\player]}] \util[\player](\otheraction[\player][]^*(\action), \naction[\player][]) - \grad[{\action[\player]}] \util[\player](\action[\player][][], \naction[\player][]) \right]  -  \grad[{\action[\player]}] \util[\player](\otheraction[\player][]^*(\action), \naction[\player][]) -  \regulparam(\action[\player][] - \otheraction[\player][]^*(\action))$ for all $\player \in \players$}{}.}\deni{This is the gradient for the regularized exploitability, not the moreau envelope in general!}
% \amy{which gives rise to a parameterized version Moreau envelope theorem}
%\deni{Good old VE exploitability w/o regularization.
This Lipschitz-smoothness of $\exploit[\regulparam]$
%of the regularized exploitability $\exploit[\regulparam]$ 
gives rise to the possibility of deriving algorithms that converge to a stationary point of $\exploit[\regulparam]$, the key idea underlying our second algorithm (\ADA; \Cref{alg:cumul_regret}).

\begin{restatable}[Parameteric Moreau Envelope Theorem]{theorem}{thmMoreauEnvelope}
\label{thm:moreau_envelope}
Given $\regulparam > 0$,
consider the parametric Moreau envelope $\exploit[\regulparam](\action) \doteq \max_{\otheraction \in \actions} \left\{\cumulregret (\action, \otheraction) - \frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2 \right\}$
and the associated proximal operator $\{\otheraction^*(\action)\} \doteq \argmax_{\otheraction \in \actions} \left\{\cumulregret (\action, \otheraction) - \frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2 \right\}$, %$\{\otheraction^*(\action)\} \doteq \argmax_{\otheraction \in \actions} \left\{\cumulregret (\action, \otheraction) - \frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2 \right\}$
where $\cumulregret$ is $\lipschitz[{\grad \cumulregret}]$-Lipschitz smooth.
%associated with the regularized cumulative regret function $\cumulregret[\regulparam]$:
% \begin{enumerate}
%     \item $\cumulregret[\regulparam]$ is $\regulparam$ strongly concave in $\otheraction$, and for all $\action \in \actionspace$, the set $\calB^*(\action)$ is a singleton.
%     \item For any SE $(\action^*, \otheraction^*)$ of $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulregret[\regulparam](\action, \otheraction)$,  $\action^*= \otheraction^*$. Additionally, $\action^*$ is a SE strategy of the outer player iff $\action^*$ is a VE of $\pgame$.\amy{this is the point i am not getting up above, but which seems important, so let's try to improve the discussion above!}
%     \item 
Then $\exploit[\regulparam](\action)$ is $\left(\lipschitz[{\grad \cumulregret}] +  \frac{\lipschitz[{\grad \cumulregret}]^2}{\regulparam} \right)$-Lipschitz-smooth, with gradients $\grad[{\action}] \exploit[\regulparam](\action) = \grad[{\action}] \cumulregret(\action, \otheraction^*(\action)) -  \regulparam(\action[][] - \otheraction[][]^*(\action))$.
% \end{enumerate}
\end{restatable}

% \begin{restatable}[Parameterized Moreau Envelope Theorem]{theorem}{lemmaLipschitzSmoothVal}
% \label{lemma:lipschitz_smooth_val}
% Given $\regulparam > 0$,
% consider the $\regulparam$-regularized exploitability %$\exploit[\regulparam](\action) \doteq \max_{\otheraction \in \actions} \cumulregret[\regulparam](\action, \otheraction)$
% and the associated solution correspondence $\{\otheraction^*(\action)\} \doteq \argmax_{\otheraction \in \actions} \cumulregret[\regulparam](\action, \otheraction)$, then
% %associated with the regularized cumulative regret function $\cumulregret[\regulparam]$:
% % \begin{enumerate}
% %     \item $\cumulregret[\regulparam]$ is $\regulparam$ strongly concave in $\otheraction$, and for all $\action \in \actionspace$, the set $\calB^*(\action)$ is a singleton.
% %     \item For any SE $(\action^*, \otheraction^*)$ of $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulregret[\regulparam](\action, \otheraction)$,  $\action^*= \otheraction^*$. Additionally, $\action^*$ is a SE strategy of the outer player iff $\action^*$ is a VE of $\pgame$.\amy{this is the point i am not getting up above, but which seems important, so let's try to improve the discussion above!}
% %     \item 
% $\exploit[\regulparam](\action)$ is $\left(\lipschitz[{\grad[\util]}] +  \frac{\lipschitz[{\grad[\util]}]^2}{\regulparam} \right)$-Lipschitz-smooth with gradients given by for all $\player \in \players$,
% $\grad[{\action[\player]}] \exploit[\regulparam](\action) =  \sum_{\player \in \players}  \left[ \grad[{\action[\player]}] \util[\player](\otheraction[\player][]^*(\action), \naction[\player][]) - \grad[{\action[\player]}] \util[\player](\action[\player][][], \naction[\player][]) \right]  -  \grad[{\action[\player]}] \util[\player](\otheraction[\player][]^*(\action), \naction[\player][]) -  \regulparam(\action[\player][] - \otheraction[\player][]^*(\action))$.
% % \end{enumerate}
% \end{restatable}




\deni{We can either keep the next two paragarphs or condense them into one, and move the definition of the projected gradient operator to the mathmatical preliminaries, and be more concise? However, I think here we have an important contribution: we are the first ones to bring into the min-max literature the use of the projected gradient operator, which allows us to obtain a nice and clearly interpretable convergence theorem, something other works are not able to do. From this stand point our proof technique is also quite novel: I did come up with the proof entirely on my own (although this is not a good argument), my point is that no one studied min-max optimization from this point of view before.}
\amy{please be sure to reiterate this point in the conclusion. about being the first to bring this idea to the min-max literature.}

Next, we formalize the definition of a stationary point.
As the exploitability $\exploit[\regulparam]$ is in general non-convex, and the optimization problem $\min_{\action \in \actions} \exploit[\regulparam] (\action)$ is constrained, 
%we need to be careful
the first-order condition $\grad \exploit[\regulparam](\action) = 0$ is not sufficient for stationarity, since a solution on the boundary of the constraint set could also be first-order stationary.
As a result, we use proximal mappings in our definition.
In particular, we reformulate the constrained exploitability minimization problem as the unconstrained minimization problem
%
% \begin{align}
$
    \min_{\action \in \R^{\numplayers \numactions}} \exploit[\regulparam](\action) + \setindic[\actions](\action).
$
% \enspace .
% \end{align}
%\deni{It is $\numplayers \numactions$ not $\numplayers \times \numactions$ because the action profile is a vector}
%
In this optimization problem, $\exploit[\regulparam]$ is continuous and Lipschitz smooth, while $\setindic[\actions]$ is continuous and convex.
Additionally, the set of solutions is non-empty.
As a result, one can solve this problem using the proximal gradient method, which, in this case, is equivalent to the projected gradient method \cite{boyd2004convex, beck2017first}.
This view of the problem as proximal minimization allows us to provide a clear definition of a first-order stationary point. 

Define the \mydef{projected gradient operator} of a function $\exploit: \actionspace \to \R$ for some step size $\learnrate[\action ][  ] > 0$ as follows:
$\gradmap[{\learnrate[\action ][  ]}][{\exploit}](\action) = \action -  \proj[\actions]\left[ \action - \learnrate[\action ][  ] \grad \exploit(\action) \right]$. The projected gradient operator is a special case of the gradient mapping operator, and a generalization
%\amy{generalization, or special case? this sentence is contradicting itself!}\deni{generalization of the plain old gradient, but special case gradient operator mapping from proximal theory.}
of the gradient that is projected back onto the feasible set $\actions$ \cite{beck2017first}.
The zeros of the projected gradient operator capture stationary points both at the boundary of the set $\actions$ and in its interior.
Indeed, $\action \in \actionspace$ is a \mydef{stationary point} of $\exploit$ if $\gradmap[{\learnrate[\action ][  ]}][{\exploit}](\action) = \zeros$.
Note that, for an action profile $\action^* \in \actionspace$ to be a VE, it is necessary that it is stationary with respect to the VE exploitability (Proposition 3, \cite{flam1994gne}).
%\footnote{We note that \citeauthor{flam1994gne} mention that this necessary condition suggests projected gradient methods could converge for pseudo-games with jointly convex constraints. Our results give an affirmative answer to their question, which has been open since 1994.}
Our goal will thus be to achieve convergence to a strategy profile $\action \in \actions$ s.t.\ $\gradmap[{\learnrate[\action ][  ]}][{\exploit[\regulparam]}](\action)
%= \left( \action -  \proj[\actions]\left[ \action - \learnrate[\action ][  ] \grad \exploit[\regulparam](\action) \right] \right)
= 0$.
\amy{so we are aiming for sufficiency, even though the condition is only necessary.}\deni{Yes gradient descent is the same}

\ADA{} (\Cref{alg:cumul_regret}) is a nested GDA algorithm, similar to those of \citeauthor{nouiehed2019solving} \cite{nouiehed2019solving} and \citeauthor{goktas2021minmax} \cite{goktas2021minmax}, with the objective function augmented by a smart regularizer.
% \if 0
% to obtain near-optimal convergence rates.
% \amy{how do we know our rates are near optimal?}\deni{So for convex-concave min-max optimization (which is a special case of a GNE) has a lowerbound of iterations of $\Omega(\nicefrac{1}{\varepsilon})$, so EDA is optimal. Unfortunately the lowerbounds for non-convex-concave optimization do not apply to our setting because the solution of a non-convex-concave min-max optimization problem does not necessarily correspond to a strategy profile which is a stationary point of the exploitability. However, since our algo's runtime is close to $\Omega(\nicefrac{1}{\varepsilon})$, I think we can in some sense argue that our algos are nearly optimal?}
% % We note that under the joint convexity assumption, the set of all feasible actions is well-defined, which we simply denote by $\actions$, i.e., $\actions = \{\action \in \actionspace \mid  \actionconstr[\player](\action[\player], \naction[\player]) \geq \zeros, \forall \player \in \players\}$
% \fi
The algorithm is reminiscent of \EDA, interleaving gradient ascent and descent steps.
The key difference is that whereas \EDA{} runs only a single step of extragradient ascent (to find a better response), \ADA{} runs multiple steps of gradient ascent to approximate a best response.
%The inner loop finds an approximate best-response to the current outer loop strategy profile, while the outer loop takes a step of gradient descent on the regularized exploitability, given this approximate best response. \sdeni{}{We note that while EDA only takes a gradient ascent step towards computing the exploitability, ADA runs an entire gradient ascent procedure in its inner loop to compute an approximation of the best-response.}
Indeed, as \Cref{thm:convergence_stationary_approx} shows, \ADA's accuracy depends on the accuracy of the best-response found.
%, which is not the case for \EDA.

\amy{if exploitability is convex, then stationarity implies Stackelberg.}


\begin{algorithm}[!h]
\caption{Augmented Descent Ascent (ADA)}
\textbf{Inputs:} $\numplayers, \util, \constr, \regulparam, \learnrate[\action], \learnrate[\otheraction], \numiters[\action], \numiters[\otheraction], \action[][][0], \otheraction[][][0]$\\
\textbf{Outputs:} $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^{\numiters[\action]}$
\label{alg:cumul_regret}
\begin{algorithmic}[1]
\For{$\iter = 0, \hdots, \numiters[\action] - 1$}
    % \For{$\player \in \players$}
    \State
    $\action[][][\iter+1] = \project[\actions] \left[\action[][][\iter] - \learnrate[\action] \left(  \grad[{\action[]}] \cumulregret(\action[][][\iter], \otheraction[][][\iter])   -  \regulparam(\action[][][\iter] - \otheraction[][][\iter]) \right) \right]$
    % \EndFor
    
    \State $\otheraction[][] = \zeros$
    
    \For{$s = 0, \hdots, \numiters[\otheraction] - 1$}
        % \For{$\player \in \players$}
        \State $\otheraction[][]  = \project[\actions] \left[ \otheraction[][][] + \learnrate[\otheraction] \left(\grad[{\otheraction}]\cumulregret(\action[][][\iter + 1], \otheraction) - \regulparam(\action[][][\iter + 1] - \otheraction[][]) \right) \right]$
    % \EndFor
    \EndFor
    
    \State $\otheraction[][][\iter + 1] =  \otheraction$
    
    \EndFor
\State \Return $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^{\numiters[\action]}$
\end{algorithmic}
\end{algorithm}


\if 0
\samy{}{To derive convergence rates for \ADA{}, we rely on two technical lemmas.
The first tells us that the inner loop can approximate the gradient of the exploitability to any desired precision.
Plugging this bound into the second lemma, we obtain a progress bound for each iteration of the outer loop.
Finally, by telescoping the inequalities in the progress lemma, we obtain our main theorem: The best iterate found by \ADA{}, as measured by the norm of the projected gradient operator, converges to a stationary point of the exploitability in all Lipschitz-smooth pseudo-games with jointly convex constraints.}
\fi

To derive convergence rates for \ADA{}, we rely on two technical lemmas. 
% \samy{Our proof technique. 
% \amy{the previous sentence said ``two technical lemmas.'' this one starts off with a proof technique. not the same thing. i think we should first say what the lemmas! and then perhaps, how you prove them.} 
The first tells us that the inner loop can approximate the gradient of the exploitability to any desired precision. More specifically, we
bound the error $\left\|\grad[\action] \exploit[\regulparam](\action[][][\iter]) - \grad[\action]\cumulregret[\regulparam](\action[][][\iter], \otheraction[][][\iter]) \right\| \leq \varepsilon$
by providing a lower bound on the number of inner loop iterations $\numiters[\otheraction]$ necessary to achieve a desired precision $\varepsilon$, for all outer loop iterations $\iter \in [\numiters[\action]]$ (\Cref{lemma:error_bound}).
% (\Cref{eq:progress_approximate_err})
% \amy{it is dangerous to reference this equation! b/c it will change before you submit the supplemental material.
The second lemma bounds the algorithm's progress at each iteration of the outer loop by relating $\varepsilon$ and $\gradmap[{\learnrate[\action ][  ]}][{\exploit[\regulparam]}](\action[\iter])$ (\Cref{lemma:progress_bound_approximate}). 
Finally, by telescoping the inequalities in the progress lemma, we obtain our main theorem: The best iterate found by \ADA{}, as measured by the norm of the projected gradient operator, converges to an approximate stationary point of the exploitability in all Lipschitz-smooth pseudo-games with jointly convex constraints. 
We further note that if the gradient of the regularized exploitability can be computed exactly, then convergence to an exact stationary point can be obtained.

\begin{restatable}[Convergence to Stationary Point of Exploitability]{theorem}{thmConvergenceStationaryApprox}
\label{thm:convergence_stationary_approx}
Suppose that \ADA{} is run on a pseudo-game $\pgame$ which satisfies \Cref{assum:main} with learning rates $\learnrate[\action] >  \frac{2}{\lipschitz[{\grad\cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad\cumulregret[\regulparam]}]^2}{\regulparam}}$ and $\learnrate[\otheraction] = \frac{1}{\lipschitz[{\cumulregret[\regulparam]}]}$, for any number of outer loop iterations $\numiters[\action] \in \N_{++}$ and for $\numiters[\otheraction] \geq \frac{2\log \left(\frac{\varepsilon}{\lipschitz[{\grad\cumulregret[\regulparam]}]} \sqrt{\frac{2 \regulparam}{c}}\right)}{\log\left(\frac{\regulparam}{\lipschitz[{\grad\cumulregret[\regulparam]}]} \right)}$ total inner loop iterations where $\varepsilon > 0$. 
Then the outputs $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^\numiters$ satisfy
%\begin{align}
% $
%     \min_{\iter = 0, \hdots, \numiters[\action] - 1} \left\|\gradmap[{\learnrate[\action ][  ]}][{\exploit[\regulparam]}](\action[][][\iter]) \right\|_2^2   \leq  \frac{1}{\learnrate[\action]  - \frac{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} }{2}} \frac{\exploit[\regulparam](\action[][][0]) - \exploit[\regulparam](\action[][][{\numiters[\action]}])}{\numiters[\action]} +  \frac{\varepsilon}{\learnrate[\action]  - \frac{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} }{2}} \left( \lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} \right)  .
% $
$
\min_{\iter = 0, \hdots, \numiters[\action] - 1} \left\|\gradmap[{\learnrate[\action ][  ]}][{\exploit[\regulparam]}](\action[][][\iter]) \right\|_2^2   \leq  \frac{1}{\frac{1}{\learnrate[\action ][  ]}  - \frac{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} }{2}} \left(\frac{\exploit[\regulparam](\action[][][0])}{\numiters[\action]} +   \varepsilon \left(\left(\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam}  + \varepsilon \right)\left(\frac{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} }{2}  -  \frac{1}{\learnrate[\action ][  ]} \right) + \lipschitz[{\cumulregret[\regulparam]}] \right)  \right) \enspace.
$
%\end{align}
% where $g = \max_{\action \in \actions} \left\|\gradmap[{\learnrate[\action ][  ]}][{\val}](\action[][][]) \right\|_2$
\end{restatable}

% in computed by ADA converges to a GNE in pseudo-games with convex exploitability, i.e., games in which the distance function to the set of GNE is convex, and jointly convex constraints, which includes but is not limited to the class of pseudo-games that EDA converges in, at a slightly slower rate of $O(\nicefrac{\log(\nicefrac{1}{\varepsilon})}{\varepsilon})$, where $\varepsilon$ is the exploitability of the game.

Note that the stationary points to which \ADA{} converges are global minima of $\exploit[\regulparam]$ iff $\exploit[\regulparam]$ is invex, in which case \ADA{} converges to a VE, and hence a GNE \cite{mishra2008invexity}.
We can also obtain faster and last iterate convergence to VE in a more restricted class of games.
A pseudo-game is said to be a $\mu$-\mydef{PL-pseudo-game} if the regularized exploitability $\exploit[\regulparam]$ satisfies the $\mu$-\mydef{projection-Polyak-Lojasiewicz (PL)} condition, i.e., the  projected gradient operator associated with $\exploit[\regulparam]$ satisfies $\nicefrac{1}{2} \left\|\gradmap[{\learnrate[\action ][  ]}][{\exploit[\regulparam]}](\action) \right\|_2^2 \geq \mu\left(\exploit[\regulparam](\action) - \min_{\action \in \actions}\exploit[\regulparam](\action) \right)$ for all $\action \in \actions$.%
\footnote{We note that this is a special case of the proximal-Polyak-Lojasiwicz condition (See Section 4, \cite{karimi2016linear}).}
A similar PL-condition for games was recently used by \citeauthor{raghunathan2019game} \cite{raghunathan2019game}, which they argued is natural.

\begin{restatable}[PL Exploitability Convergence]{theorem}{thmPLConvergence}\label{thm:pl_convergence}
Suppose \ADA{} is run on a PL-pseudo-game $\pgame$ which satisfies \Cref{assum:main} with learning rates $\learnrate[\action] \in \left[\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam}, \lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} + \frac{1}{2 \mu}\right] 
% \frac{1}{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam}}
$ and $\learnrate[\otheraction] = \nicefrac{1}{\lipschitz[{\grad \cumulregret[\regulparam]}]}$, for any number of outer loop iterations $\numiters[\action] \in \N_{++}$ and for $\numiters[\otheraction] \geq \frac{\log \left(\frac{\varepsilon}{\grad \cumulregret[\regulparam]} \sqrt{\frac{2 \regulparam}{c}}\right)}{\log\left(\frac{\regulparam}{\grad \cumulregret[\regulparam]} \right)}$ total inner loop iterations.
Then the outputs $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^\numiters$ satisfy
%\begin{align}
$
    % \exploit[\regulparam](\action[][][{\numiters[\action]}]) \leq \left[ 1  +  2\mu \left(\frac{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} }{2}   - \learnrate[\action] \right) \right]^{\numiters[\action]} \exploit[\regulparam](\action[][][0]) +   \varepsilon \left( \lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} \right).
    \exploit[\regulparam](\action[][][{\numiters[\action]}]) \leq \left[ 1  +  2\mu \left(\frac{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} }{2}   - \frac{1}{\learnrate[\action]}\right) \right]^{\numiters[\action]} \exploit[\regulparam](\action[][][0]) +    \left(\left(\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} + \varepsilon \right)\left(\frac{\lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} }{2}  -  \frac{1}{\learnrate[\action ][  ]} \right) + \lipschitz[{\cumulregret[\regulparam]}] \right)   \varepsilon  .
$
%\end{align}
% Additionally, $\lim_{\numiters[\action] \to \infty} \exploit[\regulparam](\action[][][{\numiters[\action]}]) = \varepsilon \left( \lipschitz[{\grad \cumulregret[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulregret[\regulparam]}]^2}{\regulparam} \right)$.
\end{restatable}

We note that this result also implies convergence to a VE in strongly-convex exploitability games in linear time as well, since strong convexity implies the PL-condition.


% \begin{lemma}
% Suppose that \Cref{alg:cumul_regret} is run on an input $(\numplayers, \util, \constr, \regulparam, \learnrate[\action], \learnrate[\otheraction], \numiters[\action], \numiters[\otheraction], \action[][][0])$ which satisfies \Cref{assum:main} with learning rates $\learnrate[\action] = \frac{1}{\lipschitz[{\grad[\util]}] +  \frac{\lipschitz[{\grad[\util]}]^2}{\regulparam}}$, $\learnrate[\otheraction] = \frac{1}{\lipschitz[{\cumulregret[\regulparam]}]}$ for any number of outer loop iterations $\numiters[\action] \in \N_{++}$, and for $\numiters[\otheraction] \geq \frac{\log \left(\frac{\varepsilon}{\lipschitz[\util]} \sqrt{\frac{2 \regulparam}{c}}\right)}{\log\left(\frac{\regulparam}{\lipschitz[\util]} \right)}$. Assume additionally, that Then, the outputs $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^\numiters$ satisfy
% \end{lemma}
% \begin{proof}
%     The concavity of $\cumulregret$ in $\otheraction$ can be directly inferred from the concavity of $\util[\player](\otheraction[\player], \naction[-\player])$ in $\otheraction[\player]$. We prove convex
% \end{proof}
    
    

==> Exploitability Minimization in Games and Beyond (NeurIPS)/minmax.tex <==
\section{From Exploitability Minimization To Min-Max Optimization}

In this section, we reformulate the exploitability minimization problem as a min-max optimization problem.
This reformulation is a consequence of the following observation, which is key to our analysis:
\emph{In pseudo-games for which a VE exists, e.g., pseudo-games with jointly convex constraints, the quasi-optimization problem 
% \sdeni{(with dependent constraint sets)}{} 
%\amy{wait! issue: have we said anywhere above what dependent vs. independent constraints means? if not, these parenthetical remarks are not meaningful.}\deni{We haven't better off removing!}\amy{but then where do we eventually define it? or are you just planning to just drop this distinction everywhere?}\deni{Facchinei does not make a great deal of it, and the math makes it clear, so i think we should take the same approach as well}
of minimizing exploitability, whose solutions characterize the set of GNEs, reduces to the reduces to a standard min-max optimization problem (with independent constraint sets)}, 
%namely $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulregret(\action, \otheraction)$, 
which characterizes the set of VEs, a subset of the GNEs.
% \cite{von2009optimization}.\amy{why the reference?}
This new perspective allows us to efficiently solve GNEP by computing VEs in a large class of pseudo-games as an immediate consequence of known results on the computation of saddle points in convex-concave min-max optimization problems.

Given a pseudo-game $\pgame$, we define the \mydef{regret} felt by any player $\player \in \players$ for an action $\action[\player]$  as compared to another action $\otheraction[\player]$, given the action profile $\action[-\player]$ of other players, as follows:
%
%\begin{align}
    $\regret[\player](\action[\player], \otheraction[\player]; \naction[\player]) = \util[\player](\otheraction[\player], \naction[\player]) - \util[\player](\action[\player], \naction[\player])$.
Additionally, the \mydef{cumulative regret}, or the \mydef{Nikaida-Isoda function}, $\cumulregret: \actionspace \times \actionspace \to \R$
between two action profiles $\action \in \actions$ and $\otheraction \in \actions$ across all players in a pseudo-game is given by $\cumulregret(\action, \otheraction) = \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])$.
%\enspace .
%\end{align}
%\noindent
% For notational simplicity, we will often write $\regret[\player](\action[\player], \naction[\player]) = \max_{\otheraction[\player] \in \actions[\player](\naction[\player][][][*])} \util[\player](\otheraction[\player], \naction[\player]) - \util[\player](\action[\player], \naction[\player])$
Further, the \mydef{exploitability}, or \mydef{Nikaido-Isoda \emph{potential\/} function}, $\exploit: \actionspace \to \R$ of an action profile $\action$ is defined as 
$\exploit(\action) =  \sum_{\player \in \players} \max_{\otheraction[\player] \in \actions[\player](\naction[\player])} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])$ \cite{facchinei2010generalized}.
%An alternative name for exploitability in the GNE literature is the Nikaido-Isoda potential function
Notice that the max is taken over $\actions[\player](\naction[\player])$,
%to obtain the sum of unilateral deviations, 
since a player can only deviate within the set of available strategies.

\if 0
\amy{argue that the following is true in (ordinary) games: for all $\action \in \actions$, \\
$\sum_{\player \in \players}  \max_{\otheraction[\player] \in \actionspace[\player]} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])
= \max_{\otheraction \in \actionspace} \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player]) \\$
my interpretation is that this changes the problem from a centralized one (choosing $\otheraction$) to a decentralized one (choosing $\otheraction[\player]$)}
\fi

A well-known \cite{facchinei2010generalized}%
\footnote{yet hard to exploit(!)}
result is that any unexploitable strategy profile in a pseudo-game is a GNE.
%\amy{the exploitability has to be zero, not just minimized, n'est-ce pas?}\deni{yes!!!!!}

\begin{restatable}{lemma}{lemmaNoExploitGne}
\label{lemma:no_exploit_gne}
Given a pseudo-game $\pgame$, for all $\action \in \actionspace$, $\exploit(\action) \geq 0$.
Additionally, a strategy profile $\action^* \in \actions(\action^*)$ is a GNE iff it achieves the lowerbound, i.e., $\exploit(\action^*) = 0$.
\end{restatable}

%\deni{Since you removed the fixed point correspondence description of the GNE from its definition should we do away with the quasi-optimization formulation of the GNE?, i.e., maybe we should just express it as $\min_{\action \in \actions} \exploit(\action)$?}

This lemma tells us that we can reformulate GNEP as the quasi-optimization problem of minimizing exploitability, i.e., $\min_{\action \in \actions(\action)} \exploit(\action)$.
Here, ``quasi'' refers to the fact that a solution to this problem 
%is more difficult then a traditional minimization problem, since it 
is both a minimizer of $\exploit$ \emph{and\/} a fixed point $\action^*$ s.t.\ $\action^* \in \actions(\action^*)$.\footnote{This problem could also be formulated as minimizing over the set of jointly feasible actions, i.e., $\min_{\action \in \actions} \exploit(\action)$; however, without assuming joint convexity, $\actions$ is not necessarily convex.}
Despite this reformulation of GNEP in terms of exploitability, no exploitability-minimization algorithms with convergence rate guarantees are known.
%The unexploitability(!) of exploitability seems to be due to the non-differentiability and non-convexity of exploitability, and to the difficulty imposed by the fixed-point constraint \sdeni{}{which makes it difficult to derive convergence bounds}.\amy{which one of the two mentioned difficulties make it difficult to derive convergence bounds? both? or just the fixed-point constraint?}\deni{Non-differentiability}
The unexploitability (!) of exploitability may be due to the fact that it is not Lipschitz-smooth.
%\samy{, which makes it difficult to derive convergence bounds}{}.
The key insight that allows us to obtain convergence guarantees is that we treat the GNE problem not as a quasi-minimization problem, but rather as a quasi-min-max optimization problem,
% \samy{\sdeni{}{(with dependent constraint sets)}}{} \amy{not needed here, since already a quasi problem}
namely $\min_{\action \in \actions (\action)} \exploit (\action) = \min_{\action \in \actions (\action)} \max_{\otheraction \in \actions(\action)} \cumulregret (\action, \otheraction)$.

\begin{observation}\label{obs:exploit_min_to_min_max}
Given a pseudo-game $\pgame$, for all $\action \in \actionspace$,
$\exploit(\action) = \max_{\otheraction \in \actions(\action)} \cumulregret(\action, \otheraction)$.
\end{observation}

\begin{proof}
The per-player maximum operators can be pulled out of the sum,
%in \Cref{eq:sum_max}, 
as the $\player${th} player's best action in hindsight is independent of the other players' best actions in hindsight, since the action profile $\action$ is fixed:
\begin{align*}
\exploit(\action) 
= \sum_{\player \in \players}  \max_{\otheraction[\player] \in \actions[\player](\naction[\player])} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player]) %\label{eq:sum_max}
= \max_{\otheraction \in \actions(\action)}  \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player]) %\label{eq:max_sum}
= \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
%\label{eq:sum_max}
\end{align*}
That is, the optimization problem in the $\player$th summand is independent of the optimization problem in the other summands, e.g., for any $\y \in [0, \nicefrac{1}{2}]^2$, $\max_{x_1 \in [0,1] : x_1 - y_1 \geq 0} \left\{ x_1y_1 \right\} + \max_{x_2\in [0,1] : x_2 - y_2 \geq 0} \left\{ x_2y_2 \right\} = \max_{\x \in [0, 1]^2 : \x - \y \geq \zeros } x_1y_1 + x_2y_2$.
\end{proof}

% \if 0
% \amy{DELETE, b/c this is already in the observation:}
% \begin{align}
%     \min_{\action \in \actions(\action)} \exploit(\action) &= \min_{\action \in \actions(\action)} \sum_{\player \in \players} \left[ \max_{\otheraction[\player] \in \actions[\player](\naction[\player])}  \util[\player](\otheraction[\player], \naction[\player]) - \util[\player](\action[\player], \naction[\player])  \right]\\
%     &= \min_{\action \in \actions(\action)} \max_{\otheraction \in \actions(\action)} \sum_{\player \in \players} \left[  \util[\player](\otheraction[\player], \naction[\player]) - \util[\player](\action[\player], \naction[\player])  \right]\\
%     &= \min_{\action \in \actions(\action)} \max_{\otheraction \in \actions(\action)}  \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])\\
%     &= \min_{\action \in \actions(\action)} \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
% \end{align}
% \fi
% \amy{there is a lot going on in this opt'n problem! we have dependency of $\otheraction$ on $\action$. But we also have dependency of $\action$ on itself!}
% \amy{i don't think we need to introduce the jargon of dependent and independent strategy sets.}

If we restrict our attention to VEs, a subset of GNEs, VE exploitability---hereafter exploitability, for short---is conveniently expressed as $\exploit (\action) = \max_{\otheraction \in \actions} \cumulregret (\action, \otheraction)$.
When a VE exists, e.g., in pseudo-games with jointly convex constraints, this exploitability is guaranteed to achieve the lower bound of 0 for some $\action \in \actions$.
In such cases, formulation of exploitability minimization as a quasi-min-max optimization problem reduces to a standard min-max optimization problem, 
% \amy{these parenthetical remarks are a distraction here. we have them in the first paragraph of this section, which i think should be enough.}
namely $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulregret(\action, \otheraction)$, which characterizes VEs.

This problem is well understood when $\cumulregret$ is a convex-concave objective function \cite{nemirovski2004prox, korpelevich1976extragradient, nedic2009gda, neumann1928theorie}.
Furthermore, the cumulative regret $\cumulregret$ is indeed convex-concave, i.e., convex in $\action$ and concave in $\otheraction$, in many pseudo-games of interest:
%\amy{also, does this mean the GNE is unique?}\deni{No! You would need strict-convexity-concavity.}
e.g., two-player zero-sum, $\numplayers$-player pairwise zero-sum, and a large class of monotone and bilinear pseudo-games, as well as Cournot oligopoly games.
%, to name a few (for more details, see Section 2, \cite{flam1994gne}).

Going forward, we restrict our attention to pseudo-games satisfying the following assumptions.
Lipschitz-smoothness is a standard assumption in the convex optimization literature \cite{boyd2004convex}, while joint convexity is a standard assumption in the GNE literature \cite{facchinei2010generalized}.
Furthermore, these are weaker assumptions than ones made to obtain the few known results on convergence rates to GNEs \cite{jordan2022gne}.

\begin{assumption}
\label{assum:main}
The pseudo-game $\pgame$ has joint constraints $\constr: \actionspace \to \R^\numconstrs$, and additionally,
    1.~(Lipschitz smoothness and concavity) for any player $\player \in \players$, their utility function $\util[\player]$ is $\lipschitz[{\grad[\util]}]$-Lipchitz smooth;
    %\sdeni{and concave in $\action[\player]$}{}\deni{The second part is already stated in our description of the model, so no need to state it again}
    2.~(Joint Convexity) $\constr$ is component-wise concave.
\end{assumption}

Using the simple observation that every VE of a pseudo-game is the solution to a min-max optimization problem %\samy{\sdeni{}{(with independent constraint sets)}}{}, \amy{i think/hope that by the reader knows what we mean when we say min-max opt'n problem}\deni{I think it is clear from the paragraph at bottom of page 5} 
we introduce our first algorithm (\EDA; \Cref{alg:egda_cumul_regret}), an extragradient method \cite{korpelevich1976extragradient}.
%descend on a; lower exploitability
%ascend on b; find best response
%At iteration $t$, \EDA{} takes an extragradient \emph{ascent\/} step on $\cumulregret(\action[][][\iter], \cdot)$, to obtain an iterate $\otheraction[][][\iter + 1]$ which approximates the exploitability $\exploit (\action[][][\iter])$, followed by an extragradient \emph{descent\/} step on $\cumulregret(\cdot, \otheraction[][][\iter + 1])$, which generates a new iterate $\action[\iter + 1]$ with lower exploitability than $\action[\iter]$.
The algorithm works by interleaving extragradient ascent and descent steps: at iteration $t$, given $\action[][][\iter]$, it ascends on $\cumulregret(\action[][][\iter], \cdot)$, thereby generating a better response $\otheraction[][][\iter + 1]$, and then descends on $\cumulregret(\cdot, \otheraction[][][\iter + 1])$, thereby decreasing exploitability. We combine several known results about the convergence of extragradient descent methods in min-max optimization problems to obtain the following convergence guarantees for EDA in pseudo-games.\footnote{All omitted proofs can be found in \Cref{sec_app:ommited}.} 

\begin{algorithm}[t!]
\caption{Extragradient descent ascent (EDA)}
\textbf{Inputs:} $\numplayers, \util, \actions, \learnrate,  \numiters, \action[][][0], \otheraction[][][0]$\\
\textbf{Outputs:} $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^\numiters$
\label{alg:egda_cumul_regret}
\begin{algorithmic}[1]
\For{$\iter = 0, \hdots, \numiters - 1$}
    
    \State  $\action[][][\iter + \nicefrac{1}{2}] = \project[\actions] \left[\action[][][\iter] - \learnrate[ ] \grad[{\action}] \cumulregret(\action[][][\iter], \otheraction[][][\iter]) \right]$
    
    \State  $\otheraction[][][\iter + \nicefrac{1}{2}]  = \project[\actions] \left[ \otheraction[][][\iter] + \learnrate[ ]\grad[{\otheraction}] \cumulregret(\action[][][\iter], \otheraction[][][\iter]) \right]$
    
    \State $\action[][][\iter+1] = \project[\actions] \left[\action[][][\iter ] - \learnrate[ ] \grad[{\action}] \cumulregret(\action[][][\iter + \nicefrac{1}{2}], \otheraction[][][\iter + \nicefrac{1}{2}]) \right]$
    
    \State $\otheraction[][][\iter + 1]  = \project[\actions] \left[ \otheraction[][][\iter] + \learnrate[ ]\grad[{\otheraction}] \cumulregret(\action[][][\iter + \nicefrac{1}{2}], \otheraction[][][\iter + \nicefrac{1}{2}]) \right]$

\EndFor
\State \Return $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^\numiters$
\end{algorithmic}
\end{algorithm}




\begin{restatable}[Convergence rate of EDA]{theorem}{thmedaconvergence}\label{thm:eegda}
Consider a pseudo-game $\pgame$
with convex-concave cumulative regret that satisfies \Cref{assum:main}.
Suppose that \EDA{} (\Cref{alg:egda_cumul_regret}) is run with $\learnrate[ ] < \nicefrac{1}{\lipschitz[{\grad \cumulregret}]}$, and that doing so generates the sequence of iterates $(\action[][][\iter], \otheraction[][][\iter])_{\iter = 0}^\numiters$. Let $\widebar{\action[][][\numiters]} = \nicefrac{1}{\numiters} \sum_{\iter = 1}^\numiters \action[][][\iter]$ and $\widebar{\otheraction[][][\numiters]} = \nicefrac{1}{\numiters} \sum_{\iter = 1}^\numiters \otheraction[][][\iter]$. Then the following convergence rate to a VE, i.e., to zero 
%VE
exploitability holds:
%\begin{align}
$    \max_{\otheraction \in \actions} \cumulregret(\widebar{\action[][][\numiters]}, \otheraction)  - \max_{\action \in \actions} \cumulregret(\action, \widebar{\otheraction[][][\numiters]}) \leq \nicefrac{1}{\numiters} \left( d\lipschitz[{\grad \cumulregret}] \right)$,
%\enspace ,
%\end{align}
% If EDA \Cref{alg:egda_cumul_regret} is instead run with $\learnrate[ ] < \min\{ \frac{1}{\lipschitz[{\grad \cumulregret}]} \right\}$
where $d = \max_{(\action, \otheraction) \in \actions \times \actions}  \left\| (\action, \otheraction) - (\action[][][0], \otheraction[][][0]) \right\|_2^2 $.
If, additionally, $\cumulregret$ is $\mu$-strongly-convex-$\mu$-strongly-concave, and the learning rate $\learnrate[ ] = \nicefrac{1}{4\lipschitz[\cumulregret]}$, then the following convergence bound also holds:
%\begin{align}
$    \max_{\otheraction \in \actions} \cumulregret(\widebar{\action[][][\numiters]}, \otheraction)  - \max_{\action \in \actions} \cumulregret(\action, \widebar{\otheraction[][][\numiters]}) \leq d  \nicefrac{\lipschitz[\cumulregret]^2}{\mu} \left( 1 - \nicefrac{\mu}{4 \lipschitz[\cumulregret]}\right)^\numiters$.
%\enspace .
%\end{align}
% for all $\varepsilon > 0$ and $\numiters \geq O(\nicefrac{1}{\numiters})$, $\action[][][\numiters]$ is an $\varepsilon$-GNE.
\end{restatable}

\amy{i still don't see where this fits. do you want to add something about Noah's result? maybe then it could become a standalone paragraph?} \deni{Why did it not fit in the previous paragraph? It makes a lot of sense imo?} \amy{well, it's not that it did not fit. it's just that we said, ``the following result...", and then there was this random sentence before the theorem. it broke up what was o/w a nice flow.}

\begin{remark}
%We also note that
If the players' utility functions have Lipschitz-continuous third-order derivatives, then convergence in last iterates can be obtained in $O(\nicefrac{1}{\varepsilon^2})$ iterations \cite{golowich2020eglast}.
\end{remark}

\deni{convergence occurs in last iterates (no rate) according to Korpelevich's original paper \cite{korpelevich1976extragradient}; Noah and Costis have proven a tight $\nicefrac{1}{\sqrt{T}}$ last iterate convergence recently, but \cite{nemirovski2004prox} shows convergence in average iterates in $\nicefrac{1}{{T}}$.}

Since the complexity of two-player zero-sum convex-concave games, a special case of our model, is $\Omega(\nicefrac{1}{\varepsilon})$, the iteration complexity we derive is optimal.
The exploitability minimization via \EDA{} is thus an optimal approach to GNEP in
%most pseudo-games for which computational results are known, i.e.,
convex-concave cumulative regret pseudo-games. 
Additionally, since pseudo-games generalize games, our results show that the complexity of this class of pseudo-games is the same as that of the corresponding games.

%\sdeni{An interesting observation that emerges from this new interpretation is that the computational complexity of any $\numplayers$-player (pseudo-)game is the same as that of a non-convex-concave min-max (Stackelberg) game. This observation, although interesting, does not on its own allow us to obtain convergence results to GNE (resp.\ NE) in (pseudo-)games (resp.\ games) since in general convergence to a Stackelberg equilibrium is not possible in non-convex-concave settings.}{}


\section{Pseudo-Games with Jointly Convex Constraints}\label{sec:jointly}

More generally, the exploitability minimization problem is equivalent to a non-convex-concave min-max optimization problem, i.e., cumulative regret is non-convex-concave. 
In such cases, a minimax theorem does not hold, which precludes the existence of a saddle point, making the problem much harder.
%In such cases, min-max optimization problems are best seen as Stackelberg (i.e., sequential) games, with Stackelberg equilibria as their solutions, since the order of the minimum and the maximum operators matters.
%\amy{why, when there is no minimax theorem, do we treat the game as sequential instead of simultaneous?} \deni{I think this question is not well formulated, mostly because my sentence is ill-formulated: A min-max optimization is always interpreted as a min-max Stackelberg game, because the order of operations imply an ordered game, by definition. However, in the convex-concave setting the order of the min and the max can be reversed, so that is the game is simultaneous. So the right way to formulate the sentence really is: when a minimax theorem holds the Stackelberg game can also be interpreted as a simultaneous move game.}
%\deni{I added the additional computational part bc \citeauthor{lin2020gradient} shows that with additional computation you can go from one solution concept to the other, i.e., there is a polytime reduction between the two solution concepts.} \amy{this footnote does not imply that first-order NE are inappropriate SOLUTIONS to this problem, only that they are incompatible with our proposed solution technique, which is minimizing exploitability!}
Solving
%for Stackelberg equilibria
non-convex-concave min-max optimization problems is NP-hard in general \cite{tsaknakis2021minimax}, so we instead set as our goal finding a (first-order) stationary point $\action^* \in \actions$ of the exploitability $\exploit$, i.e., a point at which first-order deviations cannot decrease the exploitability, which we show can be found in polynomial-time.
Note that any stationary point $\action^*$ of the exploitability is a $\exploit (\action^*)$-GNE of the associated pseudo-game.
%, i.e., for all players $\player \in \players$ and $\action[\player] \in \actions[\player](\naction[\player][][][*])$,  $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*]) - \exploit(\action^*) $.

\deni{I am purposefully avoiding the definition of a stationary point because the literature is a mess in terms of this in general, and in order to introduce my definition of stationary point I need to introduce my assumptions first.}

% \sdeni{$(\varepsilon, 0)$-\mydef{local Stackelberg equilibrium} of the above game. The $(\varepsilon, 0)$-local Stackelberg equilibria of $ \min_{\action \in \actionspace} \max_{\otheraction \in \actionspace } \cumulregret(\action, \otheraction)$are closely connected to \mydef{variational equilibria} of $(\numplayers, \actions, \util)$.
% Consider a strategy profile $\action^* \in \actionspace$, and suppose there exists $\varepsilon > 0$ such that $ \min_{\action \in \actionspace \cap \ball[\varepsilon][\action]} \max_{\otheraction \in \actionspace: \constr(\action, \otheraction) \geq 0} \cumulregret(\action, \otheraction) \leq \cumulregret(\action^*, \otheraction^*) \leq \max_{\otheraction \in \actionspace: \constr(\action^*, \otheraction) \geq 0} \cumulregret(\action^*, \otheraction)$, then $\action^*$ is a $\cumulregret(\action^*, \otheraction^*)$-variational equilibrium.}{} 


==> Exploitability Minimization in Games and Beyond (NeurIPS)/nonconvex.tex <==
\section{Non-Convex-Concave Stackelberg games}

Consider a min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$. When the objective function $\obj$ is non-convex-concave, the computation of Stackelberg equilibria is in general NP-hard, as the problem reduces to solving a non-convex optimization problem, and obtaining convergence guarantees in non-convex-concave settings is in general out of reach. However, in such setting one can aim to instead compute a local Stackelberg equilibrium.

\begin{definition}
A $(\varepsilon, \delta)$-\mydef{local Stackelberg equilibrium} of $(\outerset, \innerset, \obj, \constr)$ is a strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ such that:
\begin{align}
    \min_{\outer \in \outerset \cap \ball[\varepsilon][\outer]} \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer, \inner) \geq 0} \obj(\outer, \inner) \leq \obj(\outer^*, \inner^*) \leq \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer^*, \inner) \geq 0} \obj(\outer^*, \inner)
\end{align}
\end{definition}

We note that for any $\varepsilon, \delta > 0$, a $(\varepsilon, \delta)$-local Stackelberg equilibrium is guaranteed to exist whenever the payoff $\obj$, the constraints $\constr[1], \hdots, \constr[\numconstrs]$ are continuous and $\outerset, \innerset$ are non-empty and compact. We refer the reader to \citeauthor{dai2020optimality} \cite{dai2020optimality} for first and second order necessary and sufficient conditions for a strategy profile $(\outer^*, \inner^*)$ to be a $(\varepsilon, \delta)$-local Stackelberg equilibrium. When $\obj$ is concave in $\inner$, a best-response for the inner player is computable and the appropriate solution concept is the $(\varepsilon, \infty)$-local Stackelberg equilibrium, that is a strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ such that $\min_{\outer \in \outerset \cap \ball[\varepsilon][\outer]} \max_{\inner \in \innerset: \constr(\outer, \inner) \geq 0} \obj(\outer, \inner) \leq \obj(\outer^*, \inner^*) \leq \max_{\inner \in \innerset: \constr(\outer^*, \inner) \geq 0} \obj(\outer^*, \inner)$

In this paper, we will show that a $(\infty, \infty)$-Stackelberg equilibrium, i.e., (global) Stackelberg equilibrium, can be computed in polynomial time. Our results, rely on the following set of assumptions:

\begin{assumption}
    1.a.~ $\obj(\outer, \inner)$ is strictly concave in $\inner$ for all $\outer \in \outerset$\\
    1.b.~ (Polyak-Lojasiewicz condition - PL) For all $\langmult \in \R^\numconstrs_+$, $\outer \in \outerset$, and $\inner \in \innerset$, 
    % $\obj, \constr[1], \hdots, \constr[\numconstrs]$,
    $\exists \polyakconst \in \R_+$ s.t. 
    $$\nicefrac{1}{2} \left\|\grad[\outer] \obj(\outer, \inner) + \sum_{\numconstr =1}^\numconstrs \langmult[\numconstr] \grad[\outer] \constr[\numconstr](\outer, \inner)\right\| \geq \polyakconst\left( \obj(\outer, \inner) + \sum_{\numconstr =1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner) - \min_{\outer \in \outerset} \left\{\obj(\outer, \inner) + \sum_{\numconstr =1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner) \right\} \right)$$\\
    2.~ $\grad[\outer] \obj, \grad[\outer]\constr[1], \hdots, \grad[\outer]\constr[\numconstrs]$ are continuous in $(\outer, \inner)$;\\
    3.~ (Linear constraint independence qualification - LICQ) For any $\outer \in \outerset$, if $\inner^* \in \argmax_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$, then all gradients $\grad[\inner]\constr[\numconstr](\outer, \inner^*)$ such that $\constr[\numconstr](\outer, \inner^*) = 0$ are linearly independent;
    4.~ 
\end{assumption}

==> Exploitability Minimization in Games and Beyond (NeurIPS)/nsw.tex <==
\section{A Cooperative AI Application: Bargaining}

Generalized Nash equilibria have seen an increased interest due to their applicability in robot coordination. We now show another important application of generalized Nash equilibria for Cooperative AI. We study coordination games which are ubiquitous in cooperative AI. Examples of coordination games, include but are not limited to resources allocation problems, robot collaboration problems, network routing. A \mydef{coordination game} $(\numplayers, \actionspace, \disagree, \util)$ consists of $\numplayers$ players, each $\player \in \players$ characterized by an \mydef{agreement outcome set} $\actionspace[\player] \subset \R^\numactions$, \mydef{a disagreement outcome set} $\disagree[\player] \subset \R^\numactions$, and a \mydef{utility function} $\util[\player]: \actionspace \cup \disagree \to \R$ where $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player]$ and $\disagree = \bigtimes_{\player \in \players} \disagree[\player]$. Traditionally, games are studied from the lens of the Nash equilibrium, unfortunately, in coordination games Nash equilibria can highly inefficient, e.g., prisoners' dilemma, making the Nash equilibrium an undesirable solution concept for coordination problems.

An alternative solution concept for coordination games is the Nash bargaining solution, which was first introduced by \citeauthor{nash1950bargaining} \cite{nash1950bargaining} in two player bargaining, i.e., two-player coordination games. 
% The bargaining problem is an abstraction for understanding coordination problems in coordination games such as battle of the sexes \cite{}.
Nash's goal was to mathematically characterize solutions which satisfied a set of desirable axioms in Bargaining problems. In order to achieve his goal, Nash transformed his problem so that instead of showing there exists an outcome that satisfies his list of desired of axioms, he showed that there exists a distribution of utilities which satisfy his desired set of outcomes. Although this mathematical characterization was quite important in developing a theory of bargaining, as it does not allow one to compute the Nash bargaining outcome but only the utilities, it is quite hard to use in practice. We note that, the following transformation of the problems seems to have been necessary by Nash, since as we will show, the problem of computing a Nash bargaining outcome is more generally a GNE, a model introduced much after Nash's work on bargaining. 

A \mydef{Nash Bargaining game} $(\utilspace, \reserve)$ where $\utilspace \subset \R^\numplayers$ and $\reserve \in \utilspace$, consists of a set of \mydef{feasible utilities} , which is non-empty, compact and convex, and \mydef{reserves} $\reserve$. A \mydef{bargaining solution} for a bargaining problem is a function $\b: 2^{\R^\numplayers} \times \R^\numplayers \to \utilspace$,\amy{revisit} which takes as input a bargaining problem and outputs utilities for both players. Note that any coordination game $(\numplayers, \actionspace, \disagree, \util)$ can be transformed into a Nash bargaining $(\utilspace, \reserve)$ where $\utilspace = \{(\util[1](\action), \hdots, \util[\numplayers](\action)) \mid \forall \action \in \actionspace \}$, and for all players $\player \in \players$, $\reserve[\player] = \max_{\action \in \disagree} \util[\player](\action)$

A \mydef{Nash bargaining solution} is a payoff profile $\util^*$ that is a solution to the following optimization problem:
\begin{align}
    &\max_{\util \in \utilspace} & \prod_{\player \in \players} (\util[\player] - \reserve[\player])\\
    &\text{such that} & \util \geq \reserve\\
\end{align}

Note that since the set $\utilspace$ is compact, and the constraints are continuous in $\util$, the above program has a solution. Additionally, the objective is strictly quasi-concave in $\util$, the solution to the above problem is  unique.

The Nash bargaining solution is characterized by four axioms which are useful for applications in cooperative AI: 1) Pareto-optimality, 2) Symmetry, 3) Invariance to Equivalent Payoff Representations, and 4) Independence of Irrelevant We note the importance of in particular of one of these axioms.\footnote{We refer the reader to \cite{} for more information.} Pareto-optimality. A bargaining solution $\b(\utilspace, \reserve)$ is said to be \mydef{pareto-optimal} if for all $\utilspace \in 2^{\R^\numplayers}$ and $\reserve \in \R^\numplayers$, there does not exist $\util \in \utilspace$ such that for all $\player \in \players$ $\util[\player] \geq b_\player(\utilspace, \reserve)$ and $\util[k] \geq b_k(\utilspace, \reserve)$ for some $k \in \players$. Pareto-optimality is important in cooperative AI problems, since it implies that our solution is efficient for the players as a whole. Note that the Nash equilbirium is not pareto-optimal in general, leading to bad outcomes for players as a whole in general. 
% A bargaining solution $\b(\utilspace, \reserve)$ is said to be \mydef{individually rational} if for any Nash bargaing problem $(\utilspace, \reserve) \in 2^{\R^\numplayers} \times \R^\numplayers$, we have that for all players $\player \in \players$, $b_\player(\utilspace, \reserve) \geq \reserve[\player]$. Individual rationality is very desirable since otherwise the players are better off not cooperating. 

% \footnote{Formal definitions can be found \href{https://ocw.mit.edu/courses/electrical-engineering-and-computer-science/6-254-game-theory-with-engineering-applications-spring-2010/lecture-notes/MIT6_254S10_lec14.pdf}{here}}
% A bargaining solution $\b$ is said to be \mydef{symmetric} if for all $(\util, \reserve)$ such that $\util \in \utilspace$ if and only if $\pi(\util)$

% Nash has shown that the bargaining solution which satisfies 1) Pareto-optimality, 2) Symmetry, 3) Invariance to Equivalent Payoff Representations, and 4) Independence of Irrelevant Alternatives, which we posthumously call the \mydef{Nash bargaining solution}, can be computed as a solution to the following convex program:

% the set of solutions to a bargaining problem which satisfied 1) Pareto-optimality, 2) Symmetry, 3) Invariance to Equivalent Payoff Representations, and 4) Independence of Irrelevant Alternatives. 
%  For simplicity, we define the set of feasible utility profiles $\utilspace = \{(u_1, u_2) \mid \forall \allocation \in \actionspace, \util[1](\allocation) = u_1,  \util[2](\allocation) = u_2 \}$. We assume that 
 
 
Although the Nash bargaining solution provides a solution for coordination games, it does so in terms of equilibrium utilities and not in terms of the strategies. This makes it hard to use in coordination problem in practice. Hence, one might ask themselves how to reformulate such a problem from first principles with a solution given in terms of strategy profiles. 

A \mydef{Nash coordination agreement} is a strategy profile $\action^*$ such that $(\util[1](\action^*), \hdots, \util[\numplayers](\action^*))$ is the Nash bargaining solution 



% To do so, we define \mydef{a (demand) bargaining problem} $(\actionspace, \disagree, \util)$ as tuple which consists of an agreement outcome set, a disagreement outcome, and utility functions. We define a \mydef{bargaining outcome} as a function $\d: 2^\utilspace \times \utilspace \to \actionspace$ which takes as input a bargaining problem and outputs an outcome, and the \mydef{Nash bargaining outcome} as the GNE of the pseudo-game with two players, where each player $\player \in \{1, 2\}$ has a utility function $\util[\player]$, and a feasible action set $\actions[\player](\allocation[-\player])  = \{\allocation[\player] \in \actionspace[\player] \mid \util[1](\allocation) \geq \util[2](\disagree), \util[2](\allocation) \geq \util[2](\disagree)\}$. The GNE of the pseudo-game $(2, \actions, \util)$ correspond

% One\samy{}{, e.g., Amy, on her white board} might incorrectly write this as the following ill-defined optimization problem for conciseness:
% %
% \begin{align}
%     \max_{\allocation[1] \in \actions[1](\allocation[2])} \max_{\allocation[2] \in \actions[2](\allocation[1])} (\util[1](\allocation)) - \util[1](\disagree)) (\util[2](\allocation)) - \util[2](\disagree))
% \end{align}

==> Exploitability Minimization in Games and Beyond (NeurIPS)/prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

\paragraph{Notation}
We use caligraphic uppercase letters to denote sets (e.g., $\calX$);
% calligraphic uppercase letters to denote correspondences (e.g., $\calX$),
%\amy{what about correspondences? see commented out bit just here} \deni{I use caligraphic letters! Essentially mappings' letters are defined by the type of their outputs'}
bold lowercase letters to denote vectors (e.g., $\price, \bm \pi$);
bold uppercase letters to denote matrices 
%\sdeni{and vector-valued random variables (e.g., $\allocation$, $\bm \Gamma$)---which one should be clear from context;}
{(e.g., $\allocation$) and}
lowercase letters to denote scalar quantities (e.g., $x, \delta$).
%\sdeni{and uppercase letters to denote scalar-valued random variables (e.g., $X, \Gamma$)}{}.
%
We denote the $i$th row vector of a matrix (e.g., $\allocation$) by the corresponding bold lowercase letter with subscript $i$ (e.g., $\allocation[\buyer])$. 
Similarly, we denote the $j$th entry of a vector (e.g., $\price$ or $\allocation[\buyer]$) by the corresponding Roman lowercase letter with subscript $j$ (e.g., $\price[\good]$ or $\allocation[\buyer][\good]$).
%
We denote functions by a letter determined by the value of the function, e.g., $f$ if the mapping is scalar-valued, $\f$ if the mapping is vector-valued, and $\calF$ if the mapping is set-valued.
%
%We denote the vector of ones of size $\numbuyers$ by $\ones[\numbuyers]$.
%
We denote the set of integers $\left\{1, \hdots, n\right\}$ by $[n]$, the set of natural numbers by $\N$, the set of real numbers by $\R$, and the positive and strictly positive elements of a set by a $+$ and $++$ subscript, respectively, e.g., $\R_+$ and $\R_{++}$. 
% the set of positive natural numbers by $\N_+$ , the set of non-negative real numbers by $\R_+$, and the set of strictly positive real numbers by $\R_{++}$.
%
%We let $\simplex[n] = \{\x \in \R_+^n \mid \sum_{i = 1}^n x_i = 1\}$, and denote by $\simplex(A)$ the set of probability measures on the set $A$.
%
%We denote the closed epsilon ball centered at $\x$ by $\ball[\varepsilon][\x] = \{ \z \in \calZ \mid ||\z - \x || \leq \varepsilon \}$, where $\calZ$ and $\|\cdot \|$ will be clear from context.
%
%We define the indicator function of a set $\calC$ as $\setindic[\calC](\x) = 0$ if $\x \in \calC$ and $\setindic[\calC](\x) = \infty$ if $\x \notin \calC$.
%
We define the gradient $\grad[\x]: C^1(\calX) \to C^0(\calX) $ as the operator which takes as input a functional $f: \calX \to \R$, and outputs a vector-valued function consisting of the partial derivatives of $f$ w.r.t. $\x$.
%%% SPACE
%= ( x_1, \hdots, x_n)$.
%
We denote the orthogonal projection onto a set $C$ by $\project[C]$, i.e., $\project[C](\x) = \argmin_{\y \in C} \left\|\x - \y \right\|_2^2$.
Finally, we write $\setindic[\actions](\action)$ to denote the indicator function of the set $\actions$, i.e., $\setindic[\actions](\x) = 0$ if $\x \in \actions$ and $\setindic[\actions](\x) = \infty$ if $\x \notin \actions$.

\if 0
A \mydef{min-max Stackelberg game}, denoted $(\outerset, \innerset, \obj, \constr)$, is a two-player, zero-sum game, where one player, who we call the $\outer$-player (resp.\ the $\inner$-player), is trying to minimize their loss (resp.\ maximize their gain), defined by a continuous \mydef{objective function} $\obj: X \times Y \rightarrow \mathbb{R}$, by choosing a strategy from a compact \mydef{strategy set} $\outerset \subset \R^\outerdim$ (resp. $\innerset \subset \R^\innerdim$) s.t.\ $\constr(\outer, \inner) \geq 0$ where $\constr(\outer, \inner) = \left(\constr[1] (\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner) \right)^T$ with $\constr[\numconstr]: \outerset \times \innerset \to \R$, for all $\numconstr \in [\numconstrs]$. 
A strategy profile $(\outer, \inner) \in \outerset \times \innerset$ is said to be \mydef{feasible} iff $\constr[\numconstr] (\outer, \inner) \geq 0$, for all $\numconstr \in [\numconstrs]$.
The function $\obj$ maps a pair of feasible strategies taken by the players to a real value (i.e., a payoff), which represents the loss (resp.\ the gain) of the $\outer$-player (resp.\ $\inner$-player).
The relevant solution concept for Stackelberg games is the \mydef{Stackelberg equilibrium (SE)}. 
A strategy profile $\left(\outer^{*}, \inner^{*} \right) \in \outerset \times \innerset$ s.t.\ $\constr(\outer^{*}, \inner^{*}) \geq \zeros$ is a \mydef{Stackelberg equilibrium} if $\max_{\inner \in \innerset : \constr(\outer^{*}, \inner) \geq 0} \obj \left( \outer^{*}, \inner \right) \leq \obj \left( \outer^{*}, \inner^{*} \right) \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \obj \left( \outer, \inner \right)$.

A min-max game is said to be convex-concave if $\max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is convex in $\outer$, and $\obj(\outer, \inner)$ is concave in $\inner$, for all $\outer \in \outerset$.
\fi

% \begin{definition}
% A strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ is a \mydef{local Stackelberg equilibrium} of $(\outerset, \innerset, \obj, \constr)$ if there exists $\varepsilon, \delta > 0$ s.t.:
% \begin{align}
%     \min_{\outer \in \outerset \cap \ball[\varepsilon][\outer]} \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer, \inner) \geq 0} \obj(\outer, \inner) \leq \obj(\outer^*, \inner^*) \leq \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer^*, \inner) \geq 0} \obj(\outer^*, \inner)
% \end{align}

% \end{definition}
% A strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ is a \mydef{leader-local Stackelberg equilibrium} the above definition holds for $\delta = \infty$.

% A \mydef{(normal-form) game} $(\numplayers, \actionspace, \util)$ consists of  $\numplayers \in \N_+$ players. Each player $\player \in \players$ is characterized by a set of non-empty, compact, and convex strategies $\actionspace[\player]$, and a continuous utility function $\util[\player]: \actionspace \to \R$ concave in $\action[\player] \in \actionspace[\player]$ for all $\naction[\player][][][*] \in \actionspace[-\player]$ where we denote the product strategy space of all players $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player]$ and the utility function for all players by $\util(\action) =  \left(\util[1](\action), \hdots, \util[\numplayers](\action) \right)^T$. A game $(\numplayers, \actionspace, \util)$ is said to be \mydef{monotone} if for all $\action, \otheraction \in \actionspace$,
% $\sum_{\player \in \players} \left(\grad[{\action[\player]}] \util[\player](\action) - \grad[{\action[\player]}] \util[\player](\otheraction) \right)^T \left( \action - \otheraction \right) \leq 0$. A \mydef{Nash equilibrium (NE)} of a game $(\numplayers, \actionspace, \util)$ is an strategy profile $\action^* \in \actionspace$, i.e., a tuple of actions for each player, s.t.\ for all players $\player \in \players$, and for all $\action \neq \action^* \in \actionspace$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*]^*)$.

A \mydef{pseudo-game} \cite{arrow-debreu} $\pgame \doteq (\numplayers, \actionspace,  \actions, \actionconstr, \util)$ comprises $\numplayers \in \N_+$ players, each $\player \in \players$ of whom chooses an $\action[\player]$ from an action space $\actionspace[\player]$.
We denote the players' joint action space by $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player]$.
Each player $\player$ aims to maximize their continuous utility $\util[\player]: \actionspace \to \R$, which is concave in $\action[\player]$, by choosing a feasible action from a set of actions $\actions[\player](\naction[\player]) \subseteq \actionspace[\player]$ determined by the actions $\naction[\player] \in \actionspace[-\player] \subset \R^\numactions$ of the other players, where $\actions[\player]: \actionspace[-\player] \rightrightarrows  \actionspace[\player]$ is a non-empty, continuous, compact- and convex-valued action correspondence, which for convenience we represent as $\actions[\player](\naction[\player]) = \{ \action[\player] \in \actionspace[\player] \mid \actionconstr[\player][\numconstr](\action[\player], \naction[\player]) \geq \zeros, \text{ for all } \numconstr \in [\numconstrs]\}$, where for all $\player \in \players$, and $\numconstr \in [\numconstrs]$, $\actionconstr[\player][\numconstr]$ is a continuous and concave function in $\action[\player]$,\amy{in $\action[\player]$ only? what about in $\naction[\player]$}\deni{if you had concave in $\naction[\player]$, that would be a monotone game! You only need concavity in each player's action to get existence!} which defines the constraints.
We denote the product of the feasible action correspondences of all players by $\actions(\action) = \bigtimes_{\player \in \players} \actions[\player](\naction[\player])$, which we note is guaranteed to be non-empty, continuous, and compact-valued, but not necessarily convex-valued. Additionally, overloading notation, we define the set of jointly feasible strategy profiles $\actions = \{ \action \in \actionspace \mid \actionconstr[\player][\numconstr](\action) \geq \zeros, \text{ for all } \player \in \players, \numconstr \in [\numconstrs]\}$.

A two player pseudo-game is called \mydef{zero-sum} if for all $\action \in \actionspace$,
$\util[1](\action) = -\util[2](\action)$.
A pseudo-game is called \mydef{monotone} if for all $\action, \otheraction \in \actionspace$
$\sum_{\player \in \players} \left(\grad[{\action[\player]}] \util[\player](\action) - \grad[{\action[\player]}] \util[\player](\otheraction) \right)^T \left( \action - \otheraction \right) \leq 0$.
A pseudo-game is said to have \mydef{joint constraints} if there exists a function $\constr: \actionspace \to \R^\numconstrs$ s.t.\ $\constr = \actionconstr[1] = \hdots = \actionconstr[\numconstrs]$.
%, in which case the joint action correspondence is simply a set, i.e., $\actions = \{\action  \in \actionspace \mid \constr(\action) \geq \zeros\}$.
If additionally, for all $\numconstr \in [\numconstrs]$, $\constr[\numconstr](\action)$ is concave in $\action$, then we say that the pseudo-game has \mydef{jointly convex constraints}, as this assumption implies that $\actions$ is a convex set.
A \mydef{game} \cite{nash1950existence} is a pseudo-game where, for all players $\player \in \players$, $\actions[\player]$ is a constant correspondence, i.e., for all players $\player \in \players,$ $\actions[\player](\naction[\player]) = \actions[\player](\notheraction[\player])$, for all $\action, \otheraction \in \actionspace$.
Moreover, while $\actions(\action)$ is convex, for all action profiles $\action \in \actionspace$, $\actions$ is not guaranteed to be convex unless one assumes joint convexity.
\deni{We only have the following: $\action \in \actions (\action)$ and $\action \in \actions$.}
\amy{the two sets are not equivalent b/c one is a correspondence!}
%\samy{}{Note that $\action \in \actions (\action)$ implies $\action \in \actions$, for all $\action \in \actionspace$.}
%\deni{Sorry I was not clear, it is an equivalence!}

%\amy{let's delete this for space}
%\sdeni{}{We denote an strategy profile $\action \in \actionspace$, i.e., a tuple consisting of all players' strategies, as a concatenated vector of individual strategies $\action = (\action[1], \hdots, \action[\numplayers])$, write $\naction[\player]$ to refer to the strategy profile $\action$ with the $\player^{th}$ player's strategy removed, and denote by $(\action[\player]^\prime, \naction[\player])$ the strategy profile $\action$ where the $\player^{th}$ player's strategy is replaced by $\action[\player]^\prime$.}
%\deni{I am trying to make sure that it is clear that $\action^*$ is a vector a not a matrix but not sure if it is clear? Maybe this is not an important distinction.}

Given a pseudo-game $\pgame$, an $\varepsilon$-\mydef{generalized Nash equilibrium (GNE)} is strategy profile 
%$\action^* \in \actions(\action^*)$
$\action^* \in \actions(\action^*)$ s.t.\ for all $\player \in \players$ and $\action[\player] \in \actions[\player](\naction[\player][][][*])$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*]) - \varepsilon$. 
%$\util[\player](\action[\player], \naction[\player][][][*]) - \util[\player](\action^*) \leq \varepsilon$.
% \if 0
% \samy{}{$\action^* \in \actions$ s.t.\ for all $\action \in \actions$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*]) - \varepsilon$ \\
% $\action^* \in \actions$ s.t.\ for all $\action \in \actions$, $\sum_{\player \in \players} \util[\player](\action^*) \geq \sum_{\player \in \players} \util[\player](\action[\player], \naction[\player][][][*]) - \varepsilon$ \\
% $\action^* \in \actions$ s.t.\ for all $\action \in \actions$, $\sum_{\player \in \players} \left( \util[\player](\action[\player], \naction[\player][][][*]) - \util[\player](\action^*) \right) \leq \varepsilon$ \\
% $\action^* \in \actions$ s.t.\ for all $\player \in \players$ and $\action \in \actions$, $\util[\player](\action[\player], \naction[\player][][][*]) - \util[\player](\action^*) \leq \varepsilon$ \\
% $\action^* \in \actions$ s.t.\ for all $\player \in \players$ and $\action \in \actions$, $\util[\player](\action^*) \ge \util[\player](\action[\player], \naction[\player][][][*]) - \varepsilon$}
% \fi
An $\varepsilon$-\mydef{variational equilibrium (VE)} (or \mydef{normalized GNE}) of a pseudo-game is a strategy profile $\action^* \in \actions(\action^*)$ s.t.\ for all $\player \in \players$ and $\action \in \actions$, $\util[\player](\action^*) \geq  \util[\player](\action[\player], \naction[\player][][][*]) - \varepsilon$.
We note that in the above definitions, one could just as well write $\action^* \in \actions(\action^*)$ as $\action^* \in \actions$, as any fixed point of the joint action correspondence is also a jointly feasible action profile, and vice versa.
A GNE (VE) is an $\varepsilon$-GNE (VE) with $\varepsilon = 0$. 
% Note that although the set of VE of an pseudo-game is a subset of the set of GNE of the game, the converse is not true unless $\actionspace \subseteq \{\action \in \actionspace  \mid \actionconstr(\action) \geq \zeros\}$. % \deni{maybe explain why}
Under our assumptions, while GNE are guaranteed to exist in all pseudo-games by \citeauthor{arrow-debreu}'s lemma on abstract economies \cite{arrow-debreu}, VE are only guaranteed to exist in pseudo-games with jointly convex constraints 
\cite{von2009optimization}.
Note that the set of $\varepsilon$-VE of a pseudo-game is a subset of the set of the $\varepsilon$-GNE, as $\actions(\action^*) \subseteq \actions$, for all $\action^*$ which are GNE of $\pgame$.
The converse, however, is not true, unless $\actionspace \subseteq \actions$.
Further, when $\pgame$ is a game, GNE and VE coincide; we refer to this set simply as NE.

% \deni{The reason why we need the joint convexity assumption is because our goal is to compute a VE, which does not generally exist (and because projection to non-convex sets is often hard!).}

\amy{i fixed a bunch of the $\bm{a}_{-i}^*$'s manually. need a better fix to fix them everywhere!}\deni{I think I fixed them all!}\amy{did you change the macro? we need to change the macro! you you did not fix the ones in the paragraph just above this comment, which suggests that you did not change the macro?}\deni{I believe fixed now!}\amy{i didn't check the appendix. did you?}\deni{Fixed in the appendix!}

% We also define local versions of these equilibrium concepts, which are more tractable in general. A pseudo-game is simply called a \mydef{game} if for all players $\player \in \players$, $\actions(\naction[\player])$ is a constant correspondence, i.e., for all players $\player \in \players$, and strategy profiles $\action, \otheraction \in \actionspace, \actions(\naction[\player]) = \actions(\otheraction[-\player])$.


%A \mydef{local generalized Nash equilibrium (local GNE)} is an strategy profile $\action^*$ s.t.\ for all players $\player \in \players$, and $\action[\player] \in \actions[\player](\naction[\player][][][*]) \cap \ball[\varepsilon][{\action[\player]}]$, \amy{fix me!} $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*])$.
% A \mydef{local variational equilibrium (local VE) or normalized GNE} is an strategy profile $\action^*$ s.t.\ for all strategy profiles and $\action \in \actionspace \cap \ball[\varepsilon][\action]$ s.t.\ $\actionconstr(\action) \geq \zeros$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player][][][*])$. 


\if 0
A \mydef{variational inequality (VI)} problem $(\constraintset, \objs)$ given by a set $\constraintset$ and a function $\objs: \constraintset \to \R^\numconstrs$, consists of finding a solution $\x^* \in \constraintset$ s.t.\ $(\x - \x^*)^T \objs(\x^*) \geq 0.$

A \mydef{quasi-variational inequality (QVI)} problem $(\constraints, \objs)$ given by a constraint correspondence $\constraints : \constraintset \to \constraintset$ and a function $\objs: \actionspace \to \R^\numactions$, consists of finding a solution $\x^* \in \constraintset$ s.t.\ $(\x - \x^*)^T \objs(\x^*) \geq 0$, for all $\x \in \constraints(\x^*)$. 
\fi


\paragraph{Mathematical Preliminaries}
Finally, we define several mathematical concepts that are relevant to our convergence proofs.
Given $A \subset \R^\outerdim$, the function $\obj: \calA \to \R$ is said to be $\lipschitz[\obj]$-\mydef{Lipschitz-continuous} iff $\forall \outer_1, \outer_2 \in \calX, \left\| \obj(\outer_1) - \obj(\outer_2) \right\| \leq \lipschitz[\obj] \left\| \outer_1 - \outer_2 \right\|$.
If the gradient of $\obj$ is $\lipschitz[\grad \obj]$-Lipschitz-continuous, we then refer to $\obj$ as $\lipschitz[\grad \obj]$-\mydef{Lipschitz-smooth}. A function $\obj: \calX \to \R$ is said to be \mydef{invex} w.r.t.\ a function $\h: \calX \times \calX \to \calX$ if $\obj(\x) - \obj(\y) \geq \h(\x, \y)  \cdot \grad \obj(\y)$, for all $\x, \y \in \calX$.
A function $\obj: \calX \to \R$ is \mydef{convex} if it is invex w.r.t.\ $\h(\x, \y) = \x - \y$ and concave if $-\obj$ is convex.
A function $\obj: \calX \to \R$ is $\mu$-\mydef{strongly convex (SC)} if $\obj(\outer_1) \geq \obj(\outer_2) + \left< \grad[\outer] \obj(\outer_2), \outer_1 - \outer_2 \right> + \nicefrac{\mu}{2} \left\| \outer_1 - \outer_1 \right\|^2$, and $\mu$-\mydef{strongly concave} if $-\obj$ is $\mu$-strongly convex.
% \amy{move to appendix!}
% \deni{Note that the QG condition is used in the proofs.}
% \deni{We can move the last two definitions to the appendix.}

==> Exploitability Minimization in Games and Beyond (NeurIPS)/related.tex <==
%\amy{what is the background on exploitability minimization algos? who else has used them? for what games do other methods work? and are there ZERO other convergence guarantees: e.g., not even in the zero-sum case? only asymptotic guarantees?}

\paragraph{Related Work}
Following \citeauthor{arrow-debreu}'s introduction of GNE, \citeauthor{rosen1965gne} \cite{rosen1965gne} initiated the study of the mathematical and computational properties of GNE in pseudo-games with jointly convex constraints, proposing a projected gradient method to compute GNE.
Thirty years later, %after \citeauthor{rosen1965gne}'s foray into pseudo-games and their equilibria,
\citeauthor{uryas1994relax} \cite{uryas1994relax} developed the first relaxation methods for finding GNEs, which were improved upon in subsequent works \cite{Krawczyk2000relax, von2009relax}.
%Following \citeauthor{uryas1994relax}'s work,
Two other types of algorithms were also introduced to the literature: Newton-style methods \cite{facchinei2009generalized, dreves2017computing, von2012newton, izmailov2014error, fischer2016globally, dreves2013newton} and interior-point potential 
%reduction 
methods \cite{dreves2013newton}.
Many of these approaches are based on minimizing the exploitability of the pseudo-game, 
%similar to the approach taken in this paper.
but others use variational inequality\cite{facchinei2007vi, nabetani2011vi} and Lemke methods \cite{Schiro2013lemke}.

More recently, novel methods that transform GNEP to NEP were analyzed.
These models take the form of either exact penalization methods, which lift the constraints into the objective function via a penalty term %\amy{what does this mean? ``penalty type methods''?}\deni{It is when the constraints of the players are lifted to their objective function via a penalization term which is only a function of the constraints, this is as opposed to the augmented lagrangian methods which are also penalty methods but they include the dual Lagrangian variables as in the penalty term.}
\cite{facchinei2011partial, fukushima2011restricted, kanzow2018augmented, ba2020exact,  facchinei2010penalty}, or augmented Lagrangian methods \cite{pang2005quasi, kanzow2016multiplier, kanzow2018augmented, bueno2019alm}, which do the same, augmented by dual Lagrangian variables.
Using these methods, \citeauthor{jordan2022gne} \cite{jordan2022gne} provide the first convergence rates to a $\varepsilon$-GNE in monotone (resp. strongly monotone) pseudo-games with jointly affine constraints in $\tilde{O}(\nicefrac{1}{\varepsilon})$ ($\tilde{O}(\nicefrac{1}{\sqrt{\varepsilon}})$) iterations.
These algorithms, despite being highly efficient in theory, are numerically unstable in practice \cite{jordan2022gne}.
Nearly all of the aforementioned approaches concerned pseudo-games with jointly convex constraints.

Exploitability minimization has also been a valuable tool in multi-agent reinforcement learning; algorithms in this literature that aim to minimize exploitability are known as exploitability descent algorithms \cite{lockhart2019exploit}. \citeauthor{lockhart2019exploit} \cite{lockhart2019exploit} analyzed exploitability descent in two-player, zero-sum, extensive-form games with finite action spaces.
Variants of exploitability-descent have also been combined with entropic regularization and homotopy methods to solve for NE in large games \cite{gemp2021sample}.


==> GNE.tex <==
\section{Generalized Nash Equilibrium}

\begin{theorem}
Suppose that $\constraints$ is non-empty-, compact-, convex-valued, and continuous and that $\objs$ is continuous, then the VI $(\constraints, \objs)$ has at least one solution.
\end{theorem}

Additionally, just any NE is a solution to VI, we have that that every abstract economy has a GNE which is a solution to some QVI problem, the proof follows similarly.

\begin{theorem}
A strategy profile $\action^* \in \actionspace$ is a GNE of  of an abstract economy $(\numplayers, \actions, \util)$ iff it it a solution to the QVI $(\actions, - \grad[\action] \util)$.
\end{theorem}
Finally, we have the following corollary which demonstrates the existence of GNE in abstract economies


\begin{corollary}
Every abstract economy $(\numplayers, \actions, \util)$ where $\util$ is continuously differentiable has at least one Nash equilibrium.
\end{corollary}

\begin{remark}
Note that, once again, the assumption of the marginal utility being continuous can be done away (leaving us with Arrow-Debreu's lemma on abstract economies \cite{arrow-debreu}) by replacing replacing the gradient operator with the subdifferential operator, in which case $\objs$ becomes a correspondence and the VI problem becomes a \mydef{generalized QVI}, for which similar existence results holds under similar continuity assumptions.
\end{remark}



% A tuple of strategy profiles $\action^*, \otheraction^* \in \actions(\action^*)$ is said to be a \mydef{Stackelberg-best-response equilibrium (SBRE)} if for all $\player \in \players$ and for all $\action \in \actions(\action^*)$, 
% \begin{align}
%     \min_{\action \in \actionspace : \actionconstr(\action) \geq \zeros} \max_{\otheraction \in \actions(\action)} \cumulregret(\action, \otheraction) \geq  \cumulregret(\action^*, \otheraction^*) \geq \max_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction)
% \end{align}
% Intuitively, an SBRE is \deni{Wtf am I trying to say here omg.}
% or equivalently if for all $\player \in \players$
% %
% \begin{align}
%     \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \regret[\player](\action[\player]^*, \otheraction[\player] ; \naction[\player]^*) \leq 0
% \end{align}




\begin{lemma}
Consider an abstract economy $(\numplayers, \actions, \util)$. Suppose that there exists a strategy profile $\action^* \in \actions(\action^*)$ such that $\max_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction) = 0$, then $\argmax_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction) $ corresponds to the set of GNE of the abstract economy $(\numplayers, \actions, \util)$.
\end{lemma}

\begin{proof}
We have:
\begin{align}
    \max_{\otheraction \in \actions(\action^*)} \cumulregret(\action^*, \otheraction) &= 0\\
    \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \sum_{\player \in \players}  \left( \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) &= 0\\
    \sum_{\player \in \players} \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \left( \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) &= 0\\
    \sum_{\player \in \players}  \left( \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) &= 0
\end{align}
Since by \Cref{lemma:no_exploit_gne}, $\sum_{\player \in \players}  \left( \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)} \util[\player](\otheraction[\player], \naction[\player]^*) - \util[\player](\action^*) \right) \geq 0$, we must have  that for all players $\player \in \players$:
\begin{align}
    \util[\player](\action^*) = \max_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)}  \util[\player](\otheraction[\player], \naction[\player]^*)  
\end{align}

That is, $\argmax_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)}  \util[\player](\otheraction[\player], \naction[\player]^*)$ is the set of best response of player $\player \in \players$ and that $\bigtimes_{\player \in \players} \argmax_{\otheraction[\player] \in \actions[\player](\naction[\player]^*)}  \util[\player](\otheraction[\player], \naction[\player]^*)$ is the set of best-responses for all players which are fixed points of the abstract economy. 
\end{proof}


 


\begin{theorem}
Consider an abstract economy $(\numplayers, \actions, \util)$, and suppose that \Cref{assum:jointly_convex} holds and a GNE exists. Let $\cumulregret(\action, \otheraction) = \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])$, then 
any GNE of $(\numplayers, \actions, \util)$ is a Stackelberg equilibrium strategy $\action^*$ for the outer player in the following min-max game:
\begin{align}
    \min_{\action \in \actionspace: h(\action) \geq 0} \max_{\otheraction \in \actionspace:  \h(\otheraction[\player], \naction[\player]) \geq 0} \cumulregret(\action, \otheraction)
\end{align}
\end{theorem}

\begin{proof}
We have that $\min_{\action \in \actionspace: h(\action) \geq 0} \max_{\otheraction \in \actionspace:  h(\otheraction[\player], \naction[\player]) \geq 0} \cumulregret(\action, \otheraction) \geq 0$ by \Cref{lemma:no_exploit_gne}, and since a GNE $\action^* \in \actions(\action^*)$ exists, we must have that $\action^* \in \argmin_{\action \in \actionspace: \h(\action) \geq 0} \max_{\otheraction \in \actionspace:  \h(\otheraction[\player], \naction[\player]) \geq 0} \cumulregret(\action, \otheraction) $.
\end{proof}

Since games are special cases of abstract economies, we also obtain the following corollary which shows that any game is an instance of a min-max game.
\begin{corollary}
Consider a game $(\numplayers, \actionspace, \util)$ and suppose that a NE exists. Let $\cumulregret(\action, \otheraction) = \sum_{\player \in \players} \regret[\player](\action[\player], \otheraction[\player]; \naction[\player])$, then 
% the set of GNE of $(\numplayers, \actionspace, \util)$ is equal to the set of SE of $(\actionspace, \actionspace, \cumulregret, \constr)$. That is, 
any NE of $(\numplayers, \actionspace, \util)$ is a Stackelberg equilibrium strategy $\action^*$ for the outer player in the following min-max Stackelberg game:
\begin{align}
    \min_{\action \in \actionspace} \max_{\otheraction \in \actionspace} \cumulregret(\action, \otheraction)
\end{align}
\end{corollary}







==> arrow_debreu.tex <==
\section{Beyond Joint Convexity: The Example of Arrow-Debreu Markets}
Much of this paper has focused on jointly convex pseudo-games. Yet, most of the interesting applications for pseudo-games beyond this realm. We close our work with an algorithm to compute GNE beyond jointly convex domains, and provide empirical evidence of its efficacy on a canonical example of pseudo-game which is not jointly convex. We benchmark our algorithm to the most well-known algorithm to solve Arrow-Debreu markets, \mydef{t\^atonnement}, an auction-like algorithm. Before we present our results, let us recall that any pseudo-game can be written as the following ``quasi-optimization'' problem: 
$
    \min_{\action \in \actions(\action)} \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
$
Since the order of the minimum operations can be exchanged, we can decompose the outer minimization problem into $\numplayers$ minimization problems:
\begin{align}
    \min_{\action[1] \in \actions[1](\naction[1])} \min_{\action[2] \in \actions[2](\naction[2])}
    \hdots
    \min_{\action[\numplayers] \in \actions[\numplayers](\naction[\numplayers])}
    \max_{\otheraction \in \actions(\action)}  \cumulregret(\action, \otheraction)
\end{align}

The advantage of this reformulation is that it does away with the problem of simultaneously minimizing a function and solving for a fixed point problem, a problem for which no algorithms are known, and turns it into a sequential optimization problem. Even though such problems are in general NP-hard \cite{dempe2002foundations}, a local solution to such problems can often be found. This is quite desirable since very little is known on solving pseudo-games which are not jointly convex. More precisely, using the envelope theorem \cite{afriat1971envelope, milgrom2002envelope}, one can differentiate through each optimization problem to run a sequential gradient method which one would hope would converge to a stationary point of the exploitability. We note that although this approach seems very similar to that of backpropagation to obtain a direction of descent for neural network parameters, it is an inherently different method since backpropagation would make use of the implicit function theorem and the chain rule, while this approach calls for the computationally more appealing envelope theorem.

An \mydef{Arrow-Debreu (Exchange) economy model} consists of a finite set of $\numgoods$ goods, and $\numbuyers$ traders (i.e., agents/consumers). Every trader $\buyer \in \buyers$ has a set of possible consumptions $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}_+$, an endowment of goods $\consendow[\buyer] = \left(\consendow[\buyer][1], \dots, \consendow[\buyer][\numgoods] \right) \in \R^\numgoods$, a utility function $\util[\buyer]: \mathbb{R}^{\numgoods } \to \mathbb{R}$. We denote $\consumptions = \bigtimes_{\buyer \in \buyers} \consumptions[\buyer]$, and $\consendow = \left(\consendow[1], \hdots, \consendow[\numbuyers] \right)^T$. An Arrow-Debreu market is denoted by a tuple $(\util, \consumptions, \consendow)$ A \mydef{Walrassian equilibrium (WE)} is a tuple which consists of allocations $\allocation \in \R_+^{\numgoods \times \numbuyers}$, and prices $\price \in \R_+^\numgoods$ such that 1.~traders maximize utility: \\$\forall \buyer \in \buyers \ \ \ \allocation[\buyer]^*$ maximizes $\util[\buyer](\allocation[\buyer])$ over the set $\left\{ \allocation[\buyer] \ | \ \ \allocation[\buyer] \in \consumptions[\buyer] \ \ \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*  \right\}$, 2.~the markets clear and goods that are not demanded are priced at 0, i.e., $ \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  \leq \sum_{\buyer = 1}^{\numagents} \consendow[\buyer]$ and $\price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \sum_{\buyer = 1}^{\numagents} \consendow[\buyer] \right) = 0$. Any Arrow-Debreu market can be formulated as a pseudo-game whose set of GNE is equal to the of WE of the original market \cite{arrow-debreu}. We provide a new pseudo-game formulation of Arrow-Debreu markets, whose exploitability is much easier to differentiate. 
	
\begin{theorem}
Consider the Arrow-Debreu market $(\util, \consumptions, \consendow)$, then any WE $(\allocation^*, \price^*)$, corresponds to a Stackelberg equilibrium strategy of the outer player $(\allocation^*, \price^*)$ in the following convex-concave min-max Stackelberg game:
\begin{align}
    \min_{(\allocation, \price) \in \consumptions \times \simplex[\numgoods] : \allocation \price \leq \consendow \price} \max_{(\Y, \q) \in \consumptions \times \simplex[\numgoods] : \Y \price \leq \consendow \price} \left(\q - \price \right)^T \left(  \sum_{\buyer \in \buyers} \allocation[\buyer] - \sum_{\buyer \in \buyers} \consendow[\buyer] \right) + \sum_{\buyer \in \buyers} (\consendow[\buyer] \cdot \price ) \left( \log(\util[\buyer](\y_{\buyer}))  - \log(\util[\buyer](\allocation[\buyer])) \right)
\end{align}
\end{theorem}


\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_arrow_debreu_linear.png}
         \caption{Linear Arrow-Debreu Market}
         \label{fig:linear_ad}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_arrow_debreu_cd.png}
         \caption{Cobb-Douglas Arrow-Debreu Market}
         \label{fig:cd_ad}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graphs/exploit_arrow_debreu_leontief.png}
         \caption{Leontief Arrow-Debreu Market}
         \label{fig:leontief_ad}
     \end{subfigure}
        \caption{Convergence of sequential exploitability descent in Arrow-Debreu markets.
        % for \ref{fig:phase_zero_sum_affine} a game with one action, and 
        }
        \label{fig:ad}
\end{figure*}



==> checklist.tex <==
% \section*{Submission of papers to NeurIPS 2022}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Appendix A}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, details are discussed in conclusion, and experiments sections.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Assumptions are summarized in \Cref{assum:main}}
        \item Did you include complete proofs of all theoretical results? 
    \answerYes{Yes, all proofs can be found in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, code repo can be found here: \coderepo.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details can be found in section 5 and Appendix A.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{For experiments run multiple times, i.e., zero-sum convex constraints, exploitability always reached zero, and there was hence no error to report in all randomly initialized examples.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details can be found in Appendix A.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Details can be found in Appendix A}
  \item Did you mention the license of the assets?
    \answerYes{Details can be found in Appendix A}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> nonconvex.tex <==
\section{Non-Convex-Concave Stackelberg games}

Consider a min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$. When the objective function $\obj$ is non-convex-concave, the computation of Stackelberg equilibria is in general NP-hard, as the problem reduces to solving a non-convex optimization problem, and obtaining convergence guarantees in non-convex-concave settings is in general out of reach. However, in such setting one can aim to instead compute a local Stackelberg equilibrium.

\begin{definition}
A $(\varepsilon, \delta)$-\mydef{local Stackelberg equilibrium} of $(\outerset, \innerset, \obj, \constr)$ is a strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ such that:
\begin{align}
    \min_{\outer \in \outerset \cap \ball[\varepsilon][\outer]} \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer, \inner) \geq 0} \obj(\outer, \inner) \leq \obj(\outer^*, \inner^*) \leq \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer^*, \inner) \geq 0} \obj(\outer^*, \inner)
\end{align}
\end{definition}

We note that for any $\varepsilon, \delta > 0$, a $(\varepsilon, \delta)$-local Stackelberg equilibrium is guaranteed to exist whenever the payoff $\obj$, the constraints $\constr[1], \hdots, \constr[\numconstrs]$ are continuous and $\outerset, \innerset$ are non-empty and compact. We refer the reader to \citeauthor{dai2020optimality} \cite{dai2020optimality} for first and second order necessary and sufficient conditions for a strategy profile $(\outer^*, \inner^*)$ to be a $(\varepsilon, \delta)$-local Stackelberg equilibrium. When $\obj$ is concave in $\inner$, a best-response for the inner player is computable and the appropriate solution concept is the $(\varepsilon, \infty)$-local Stackelberg equilibrium, that is a strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ such that $\min_{\outer \in \outerset \cap \ball[\varepsilon][\outer]} \max_{\inner \in \innerset: \constr(\outer, \inner) \geq 0} \obj(\outer, \inner) \leq \obj(\outer^*, \inner^*) \leq \max_{\inner \in \innerset: \constr(\outer^*, \inner) \geq 0} \obj(\outer^*, \inner)$

In this paper, we will show that a $(\infty, \infty)$-Stackelberg equilibrium, i.e., (global) Stackelberg equilibrium, can be computed in polynomial time. Our results, rely on the following set of assumptions:

\begin{assumption}
    1.a.~ $\obj(\outer, \inner)$ is strictly concave in $\inner$ for all $\outer \in \outerset$\\
    1.b.~ (Polyak-Lojasiewicz condition - PL) For all $\langmult \in \R^\numconstrs_+$, $\outer \in \outerset$, and $\inner \in \innerset$, 
    % $\obj, \constr[1], \hdots, \constr[\numconstrs]$,
    $\exists \polyakconst \in \R_+$ s.t. 
    $$\nicefrac{1}{2} \left\|\grad[\outer] \obj(\outer, \inner) + \sum_{\numconstr =1}^\numconstrs \langmult[\numconstr] \grad[\outer] \constr[\numconstr](\outer, \inner)\right\| \geq \polyakconst\left( \obj(\outer, \inner) + \sum_{\numconstr =1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner) - \min_{\outer \in \outerset} \left\{\obj(\outer, \inner) + \sum_{\numconstr =1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner) \right\} \right)$$\\
    2.~ $\grad[\outer] \obj, \grad[\outer]\constr[1], \hdots, \grad[\outer]\constr[\numconstrs]$ are continuous in $(\outer, \inner)$;\\
    3.~ (Linear constraint independence qualification - LICQ) For any $\outer \in \outerset$, if $\inner^* \in \argmax_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$, then all gradients $\grad[\inner]\constr[\numconstr](\outer, \inner^*)$ such that $\constr[\numconstr](\outer, \inner^*) = 0$ are linearly independent;
    4.~ 
\end{assumption}

==> nsw.tex <==
\section{A Cooperative AI Application: Bargaining}

Generalized Nash equilibria have seen an increased interest due to their applicability in robot coordination. We now show another important application of generalized Nash equilibria for Cooperative AI. We study coordination games which are ubiquitous in cooperative AI. Examples of coordination games, include but are not limited to resources allocation problems, robot collaboration problems, network routing. A \mydef{coordination game} $(\numplayers, \actionspace, \disagree, \util)$ consists of $\numplayers$ players, each $\player \in \players$ characterized by an \mydef{agreement outcome set} $\actionspace[\player] \subset \R^\numactions$, \mydef{a disagreement outcome set} $\disagree[\player] \subset \R^\numactions$, and a \mydef{utility function} $\util[\player]: \actionspace \cup \disagree \to \R$ where $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player]$ and $\disagree = \bigtimes_{\player \in \players} \disagree[\player]$. Traditionally, games are studied from the lens of the Nash equilibrium, unfortunately, in coordination games Nash equilibria can highly inefficient, e.g., prisoners' dilemma, making the Nash equilibrium an undesirable solution concept for coordination problems.

An alternative solution concept for coordination games is the Nash bargaining solution, which was first introduced by \citeauthor{nash1950bargaining} \cite{nash1950bargaining} in two player bargaining, i.e., two-player coordination games. 
% The bargaining problem is an abstraction for understanding coordination problems in coordination games such as battle of the sexes \cite{}.
Nash's goal was to mathematically characterize solutions which satisfied a set of desirable axioms in Bargaining problems. In order to achieve his goal, Nash transformed his problem so that instead of showing there exists an outcome that satisfies his list of desired of axioms, he showed that there exists a distribution of utilities which satisfy his desired set of outcomes. Although this mathematical characterization was quite important in developing a theory of bargaining, as it does not allow one to compute the Nash bargaining outcome but only the utilities, it is quite hard to use in practice. We note that, the following transformation of the problems seems to have been necessary by Nash, since as we will show, the problem of computing a Nash bargaining outcome is more generally a GNE, a model introduced much after Nash's work on bargaining. 

A \mydef{Nash Bargaining game} $(\utilspace, \reserve)$ where $\utilspace \subset \R^\numplayers$ and $\reserve \in \utilspace$, consists of a set of \mydef{feasible utilities} , which is non-empty, compact and convex, and \mydef{reserves} $\reserve$. A \mydef{bargaining solution} for a bargaining problem is a function $\b: 2^{\R^\numplayers} \times \R^\numplayers \to \utilspace$,\amy{revisit} which takes as input a bargaining problem and outputs utilities for both players. Note that any coordination game $(\numplayers, \actionspace, \disagree, \util)$ can be transformed into a Nash bargaining $(\utilspace, \reserve)$ where $\utilspace = \{(\util[1](\action), \hdots, \util[\numplayers](\action)) \mid \forall \action \in \actionspace \}$, and for all players $\player \in \players$, $\reserve[\player] = \max_{\action \in \disagree} \util[\player](\action)$

A \mydef{Nash bargaining solution} is a payoff profile $\util^*$ that is a solution to the following optimization problem:
\begin{align}
    &\max_{\util \in \utilspace} & \prod_{\player \in \players} (\util[\player] - \reserve[\player])\\
    &\text{such that} & \util \geq \reserve\\
\end{align}

Note that since the set $\utilspace$ is compact, and the constraints are continuous in $\util$, the above program has a solution. Additionally, the objective is strictly quasi-concave in $\util$, the solution to the above problem is  unique.

The Nash bargaining solution is characterized by four axioms which are useful for applications in cooperative AI: 1) Pareto-optimality, 2) Symmetry, 3) Invariance to Equivalent Payoff Representations, and 4) Independence of Irrelevant We note the importance of in particular of one of these axioms.\footnote{We refer the reader to \cite{} for more information.} Pareto-optimality. A bargaining solution $\b(\utilspace, \reserve)$ is said to be \mydef{pareto-optimal} if for all $\utilspace \in 2^{\R^\numplayers}$ and $\reserve \in \R^\numplayers$, there does not exist $\util \in \utilspace$ such that for all $\player \in \players$ $\util[\player] \geq b_\player(\utilspace, \reserve)$ and $\util[k] \geq b_k(\utilspace, \reserve)$ for some $k \in \players$. Pareto-optimality is important in cooperative AI problems, since it implies that our solution is efficient for the players as a whole. Note that the Nash equilbirium is not pareto-optimal in general, leading to bad outcomes for players as a whole in general. 
% A bargaining solution $\b(\utilspace, \reserve)$ is said to be \mydef{individually rational} if for any Nash bargaing problem $(\utilspace, \reserve) \in 2^{\R^\numplayers} \times \R^\numplayers$, we have that for all players $\player \in \players$, $b_\player(\utilspace, \reserve) \geq \reserve[\player]$. Individual rationality is very desirable since otherwise the players are better off not cooperating. 

% \footnote{Formal definitions can be found \href{https://ocw.mit.edu/courses/electrical-engineering-and-computer-science/6-254-game-theory-with-engineering-applications-spring-2010/lecture-notes/MIT6_254S10_lec14.pdf}{here}}
% A bargaining solution $\b$ is said to be \mydef{symmetric} if for all $(\util, \reserve)$ such that $\util \in \utilspace$ if and only if $\pi(\util)$

% Nash has shown that the bargaining solution which satisfies 1) Pareto-optimality, 2) Symmetry, 3) Invariance to Equivalent Payoff Representations, and 4) Independence of Irrelevant Alternatives, which we posthumously call the \mydef{Nash bargaining solution}, can be computed as a solution to the following convex program:

% the set of solutions to a bargaining problem which satisfied 1) Pareto-optimality, 2) Symmetry, 3) Invariance to Equivalent Payoff Representations, and 4) Independence of Irrelevant Alternatives. 
%  For simplicity, we define the set of feasible utility profiles $\utilspace = \{(u_1, u_2) \mid \forall \allocation \in \actionspace, \util[1](\allocation) = u_1,  \util[2](\allocation) = u_2 \}$. We assume that 
 
 
Although the Nash bargaining solution provides a solution for coordination games, it does so in terms of equilibrium utilities and not in terms of the strategies. This makes it hard to use in coordination problem in practice. Hence, one might ask themselves how to reformulate such a problem from first principles with a solution given in terms of strategy profiles. 

A \mydef{Nash coordination agreement} is a strategy profile $\action^*$ such that $(\util[1](\action^*), \hdots, \util[\numplayers](\action^*))$ is the Nash bargaining solution 



% To do so, we define \mydef{a (demand) bargaining problem} $(\actionspace, \disagree, \util)$ as tuple which consists of an agreement outcome set, a disagreement outcome, and utility functions. We define a \mydef{bargaining outcome} as a function $\d: 2^\utilspace \times \utilspace \to \actionspace$ which takes as input a bargaining problem and outputs an outcome, and the \mydef{Nash bargaining outcome} as the GNE of the pseudo-game with two players, where each player $\player \in \{1, 2\}$ has a utility function $\util[\player]$, and a feasible action set $\actions[\player](\allocation[-\player])  = \{\allocation[\player] \in \actionspace[\player] \mid \util[1](\allocation) \geq \util[2](\disagree), \util[2](\allocation) \geq \util[2](\disagree)\}$. The GNE of the pseudo-game $(2, \actions, \util)$ correspond

% One\samy{}{, e.g., Amy, on her white board} might incorrectly write this as the following ill-defined optimization problem for conciseness:
% %
% \begin{align}
%     \max_{\allocation[1] \in \actions[1](\allocation[2])} \max_{\allocation[2] \in \actions[2](\allocation[1])} (\util[1](\allocation)) - \util[1](\disagree)) (\util[2](\allocation)) - \util[2](\disagree))
% \end{align}
